Intrinsic Point of Interest Discovery from Trajectory Data

This paper presents a framework for intrinsic point of interest discovery from trajectory databases. Intrinsic points of interest are regions of a geospatial area innately defined by the spatial and temporal aspects of trajectory data, and can be of varying size, shape, and resolution. Any trajectory database exhibits such points of interest, and hence are intrinsic, as compared to most other point of interest definitions which are said to be extrinsic, as they require trajectory metadata, external knowledge about the region the trajectories are observed, or other application-specific information. Spatial and temporal aspects are qualities of any trajectory database, making the framework applicable to data from any domain and of any resolution. The framework is developed under recent developments on the consistency of nonparametric hierarchical density estimators and enables the possibility of formal statistical inference and evaluation over such intrinsic points of interest. Comparisons of the POIs uncovered by the framework in synthetic truth data to thousands of parameter settings for common POI discovery methods show a marked improvement in fidelity without the need to tune any parameters by hand.

==> ClusterTree POIs/includes/definitions.tex <==
\newenvironment{enumNoSpace}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}{\end{enumerate}
}

\newtheorem{mydef}{Definition}
\AfterEndEnvironment{mydef}{\noindent\ignorespaces}

\newenvironment{myalg}[1]
  {\mdfsetup{
    frametitle={\colorbox{white}{\space#1\space}},
    innertopmargin=0pt,
    frametitleaboveskip=-\ht\strutbox,
    frametitlealignment=\center
    }
  \begin{mdframed}%
  }
  {\end{mdframed}}

\def\aand{{\rm and}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Q}{\mathbf{Q}}
%\newcommand{\U}{\mathbf{U}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\Pm}{\mathbf{P}}
\def\emt{\pmb{\emptyset}}
\def\eps{\pmb{\varepsilon'}}
\def\epsa{\pmb{\varepsilon_{\bf a}'}}
\def\epsb{\pmb{\varepsilon_{\bf b}'}}
\def\epsu{\pmb{\varepsilon_{\bf u}'}}
\def\and{{\rm and}}
%\def\lft{{\rm (}}
\def\o{{\rm o}}
%\def\rt{{\rm )}}
\def\for{{\rm for}}
\def\lgl{\pmb{\langle}\,}
\def\rgl{\,\pmb{\rangle}}
\renewcommand{\E}{\pmb{\mathbb{E}}}
\newcommand{\R}{\pmb{\mathbb{R}}}
\newcommand{\topic}{\subsection*}

\newenvironment{Figure}
  {\par\medskip\noindent\minipage{\linewidth}}
  {\endminipage\par\medskip}

==> ClusterTree POIs/intrinsic.tex <==
This section provides preliminary information about the POI discovery problem, and provides context and definitions for this work. It then formally defines a POI and (subsequently) an intrinsic POI, and the framework their discovery. 
\subsection{Preliminaries} 
We consider a trajectory database of discrete, time-indexed spatial data having at least the 3-tuple of attributes
$$(\texttt{<object id>}, \texttt{<spatial component>}, \texttt{<temporal component>})$$ 
This minimal amount of information implies a {\it trajectory} for an object of the form: 
\begin{equation}\label{eq:1}
	T = p_1 \xrightarrow[]{\Delta t_1} p_2 \xrightarrow[]{\Delta t_2} \dots \xrightarrow[]{\Delta t_{n-1}} p_n
\end{equation}
where $p_1, p_2, ..., p_n$ are chronologically ordered spatial coordinates. In the geographical sense, these spatial components are often defined by a \texttt{<latitude>} and \texttt{<longitude>} pair, but in practice could be from any coordinate system. 
Such representations require {\it trajectory pattern mining} techniques~\cite{zheng2015trajectory}, or techniques that seek to mine common spatiotemporal patterns across trajectories to assert significance over areas where trajectory patterns emerge. Mined patterns in trajectories are often referred to as {\it mobility patterns}, characterizing some specific trajectory quality of interest, such as heading, stopping rate, velocity, rotation, curvature, or shape~\cite{buchin2011segmenting}. Such mobility patterns exhibit properties that make the formal retrieval of significant areas challenging. For example, if the timespan of an observed trajectory is long, the processes driving the mobility pattern may be non-stationary (e.g. road traffic that changes due to construction, or congestion effects due to time of day shifts in the work schedule). There may also be paths of objects that are transient (some areas are never traveled to more than once). Furthermore, the spatial components in trajectory data often have a high degree of autocorrelation, breaking assumptions of independence~\cite{figueiredo2016tribeflow}. A variety of models have been proposed to handle thee situations, largely focusing on estimating {\it individual} trajectory statistics under these assumptions. This includes, for examples, adaptive Kalman filters for vehicle navigation~\cite{hu2009adaptive}, state-space models~\cite{gindele2010probabilistic}, and trajectory path uncertainty models~\cite{trajcevski2009continuous}.

% To systematically address all of these assumptions is impractical, and 
The knowledge mined from individual trajectories says little of the {\it macroscopic patterns driving such trajectory observations}. Rather than focusing on the statistics of individual trajectories,
{\em collective models} preprocess the trajectory data to extract characteristics across a swath of trajectories. Such preprocessing is desirable, as it discards highly autocorrelated data representing redundant information in favor of aggregating trajectory positions into observations of significance. Examples of this preprocessing scheme include extracting ``semantically enriched'' points that intersect known geographical regions~\cite{alvares2007model}, aggregating trajectory positions as stay points using supplied spatial and/or temporal thresholds~\cite{zheng2010geolife}, or processing trajectory data into groups using some  convex combination of spatial, temporal, and semantic similarity kernels~\cite{liu2013todmis, ying2011semantic}. 

In a collective model, we refer to the `important' or semantically meaningful data samples aggregated from trajectory points as {\it exemplar positions}, or simply, {\it exemplars}:
%%% ASK MATT
\begin{mydef} {\bf Exemplar}\\
	Consider a sample of $n$ discrete points $X_n \subset \mathbb{R}^d$ that 
	constitute a trajectory $T$. 
	Define an aggregation function $\alpha : \mathcal{P}(X_n) \mapsto \mathbb{R}^d$ 
	that maps any subset of points (e.g. a trajectory segment) in $T$ to a set of {\bf exemplar} positions $\Sigma \subset \mathbb{R}^d$. 
\end{mydef}
\noindent
%% Matt I do not understand the iid assumption. How can Sigma be iid samples of f? Sigma is the range of f. Moreover each element in Sigma is the result of some aggregation of points in \mathcal{X}, so I don't
%% the sampling thing. Do all elements in mathcal{X} need to be iid? No since they can be aggregated into
%% trajectories and trajectory point locations are not iid. i've commented out that assumption.
The aggregation function of choice depends on the intent of the analysis. For example, consider an urban environmental study that defines $\alpha$ as a mapping of some isolated trajectory {\it segment} $\{p_k, p_{k+1}, ..., p_{k+l}\}$ to the mean coordinate of the segment if the speed of the object traveling from $p_k$ to $p_{k+l}$ exceeds a certain threshold. Groups of these exemplar positions may determine ``high-emission'' zones in a city~\cite{baluja2016reducing}. Alternatively, if the traffic is made of pedestrians, such groups may represent tourist attraction areas, the popularity of which are useful for LBS applications~\cite{zheng09}. 
It is not difficult to find this type of trajectory preprocessing in geospatial applications, and the grouping of them is foundational to countless tasks in trajectory mining~\cite{zheng2010geolife, alvares2007model, liu2012tra, zhou07, zheng09, ying2011semantic}. We generalize this preprocessing step by referring to it as ``exemplar extraction.''

An important aspect of exemplar extraction is to choose an aggregation function that befits the intent of the analyst and thus satisfies a study's interpretation of ``interesting.'' This is inevitably application-specific, and the proposed framework is agnostic to the specific form of aggregation used, thus it is irrelevant to bestow a particular interpretation of what ``interesting" means. We consider a more concrete and practical definition using a popular type of aggregation in Section \ref{sec:experiments_and_discussion}. 
%These groups of exemplary points effectively represent the collections of similar mobility pattern of interest within an area. Under this notion of a location, the important aspect of the data is not as much the trajectory data of the form in Equation~\ref{eq:1}, but the actual format of the data {\em used to train discriminative models}:
%\begin{equation}\label{eq:2}
%T_{\ell} = \ell_1 \xrightarrow[]{\Delta t_1} \ell_2 \xrightarrow[]{\Delta t_2} \dots \xrightarrow[]{\Delta t_{m-1}} \ell_m
%\end{equation}


%This matches the intent of the paper with the particular methodology used; clustering is often quoted as a useful tool for for data exploration~\cite{}, knowledge discovery~\cite{guyon2009clustering}, and to identify some innate `structure' within  the data being analyzed~\cite{}. 


% Matt - not for this paper, but a figure of this would be great (going from trajectories to subtrajectories to locations)
% - Noted 
% Location discovery approaches, however, seldom rely only on the fundamental spatial and temporal aspects of the data, limiting the generalizability of the methods used or rendering approaches to be problem-specific. 
% Matt, the first sentence says trajectories -> locations depend on more than temporal and position data.
% but then we say, in this paper, that we assume the problem has already been solved (that we 
% already have exemplars). Then we discuss how exemplars lead to groupings of exemplars that mean... what?
% It reads like exemplars == positions. Are "semantically enriched points" exemplars? 
% I think these two paragraphs need to be rewritten for clarity
% - Fixed; formally defined an exemplar sort of

% For example, in the geospatial sense, if groups or `convoys' of vehicles that travel to similar locations (e.g. vehicle 1 travels from $\ell_2 \xrightarrow{} \ell_1 \xrightarrow{} \ell_3$ and vehicle 2 travels $\ell_2 \xrightarrow{} \ell_4 \xrightarrow{} \ell_3$, there is evidence that these vehicle may be related, as they had a common beginning and ending location. Despite this simple idea that {\em completely predetermines} the input of many state-of-the-art models, often enough such models use some potentially biased gazeteer to define what and where a `location' is. 

% --------------------------------------------------------------------
% --------------------- DEFINING A POI ---------------------------------
% --------------------------------------------------------------------
%% Matt general comment, use high density or high-density consistently everywhere. 

\begin{figure*}
 	\includegraphics[width=\textwidth, height=5.95cm]{ctree5}
 	\caption{Illustrating the cluster tree hierarchy and its interpretation of POIs. Consider an estimated density (right panel) of exemplar positions extracted from trajectories in a geospace (middle, bottom panel). A POI is a geospatial region inhabited by exemplar positions at some density threshold $\lambda$, with the number of the POIs extracted depend on this scale parameter setting (left panel). Higher $\lambda$ limits a POI to being specific and small, and could cause POIs to be manifested by random noise or be overfitted to a particular set of observations. Low $\lambda$ defines POIs as very broad areas of low exemplar position density. The cluster tree hierarchy (left panel) summarizes the set of exemplar positions representing a POI at every density threshold, thus capturing the entire collection of POIs over a common area (middle panel, upper layers). }
 	\label{fig:ctree}
\end{figure*}

\subsection{Defining a point of interest}\label{sec:definition}
Under the premise that exemplars represent meaningful aggregations of observations from a trajectory data source, it is natural to define a POI as {\em a region of exemplars}. We seek a definition of such regions with a statistical (rather than heuristic) foundation as a means of reflecting the naturally occurring structure within the data. Towards this end, we define a POI as a {\em contiguous, high density region of exemplars}. 

To formalize this definition, we follow the notation of Chaudhuri et. al~\cite{chaudhuri2010rates}. Let $\mathcal{X}$ be a subset of $\mathbb{R}^d$ and define a {\em path} as a function $P : [0,1] \to S$ where $S \subset \mathcal{X}$. Also denote the equivalence relation $C$ as {\em connected}, where $xCy$ iff $P(0) = x$ and $P(1) = y$. Then $C$ partitions $S$ into {\it connected components} or {\em clusters}. Each component represents an area of high density and is called a {\em high density cluster}:
\begin{mydef} {\bf High density clusters}\\
For a density function $f$ on $\mathbb{R}^d$, consider a partitioning:
	\begin{equation}\label{eq:poi}
		\{ x : f(x) \geq \lambda \}\text{, for some }\lambda > 0
	\end{equation}
where $\lambda$ is called the level, or high density threshold, parameter. Then all maximally connected components in this set are {\bf high density clusters} at density level $\lambda$. 
\end{mydef}
We relate this formal definition to the trajectory mining domain with the following definition of a point of interest, defined over {\em a extracted set of exemplars}. 
\begin{mydef} {\bf Point of interest}\\
Given a set of $m$ exemplars $\{\varepsilon_1, \varepsilon_2, \dots, \varepsilon_m\} \in \Sigma$ and a fixed ``scale'' or resolution $\lambda$, each high density cluster of such exemplars forms a {\bf point of interest} at the density level $\lambda$. 
\end{mydef}
The sets of high density clusters across all values of $\lambda$ forms a hierarchy often referred to as the {\bf cluster tree} of the density $f$~\cite{chaudhuri2010rates, chen2016statistical}. 
A hierarchical definition of locations is common~\cite{zheng09} and matches the intuitive interpretation of a POI. For example, not only may a particular restaurant in a mall food court be a POI, but the food court itself may also be considered a POI, as well as entire mall may be yet another POI. The cluster tree conceptualization formalizes a POI as a maximally connected set of exemplars falling along a higher density area, implying such areas are `significant,' and that such connected exemplars may be related.    

A visualization of hierarchical POIs and a dendrogram of the corresponding cluster tree is provided in Figure~\ref{fig:ctree}. The middle figure demonstrates a high-level view of what a set of trajectories might look like, with the colored dots in the left and middle figures representing exemplars. The right figure demonstrates a density estimate of the positions of these exemplars. That is, when these exemplars are very close to each other, they're said {\em to have a high density and are thought to be related}, constituting a POI---the scale of the density depends on the analysis at hand. A sufficiently low density threshold $\lambda_0$ will designate every exemplar as one POI.

From this definition, it may seem that any arbitrary density estimator may be used to find high-density clusters: simply estimate the density of every point by kernel density estimation (KDE), and then iterate through all possible values of $\lambda$ that create distinct high-density clusters. Yet not every estimation will produce the same hierarchy---different kernels (and kernel bandwidths) may result in a completely different hierarchy of high-density clusters, and by extension, a different set of POIs.  
From the cluster tree perspective, the ideal kernel $f_n$ is one that is uniformly consistent (i.e. $\sup_x{\lvert f_n(x) - f(x) \rvert} \to 0 \text{ as } n \to \infty$) from a given sample $X_n$. In this case,  a model could be fitted with the appropriate kernel and bandwidth parameter, and the would KDE furnish a continuous surface from which a cluster tree and its high-density clusters can be derived~\cite{chen2016statistical}. The main issue is that the set of all high-density clusters is not easy to compute for typical density estimates of $f$~\cite{chaudhuri2010rates} and generally require a significant amount of memory to store. This computational inefficiency limits usability for large trajectory datasets, often observed over wide geographical areas and over long periods of time. 
% Furthermore, even if a uniformly consistent KDE may be plausible in theory, there is not always guidance with how to configure the parameter settings of such an approach, leading to resulting density inspiring questions as to what such a statistical estimation truly reveals about the underlying space, and whether such information is {\it useful} to the application at hand. The choice of the bandwidth or `influence' parameter may not be obvious~\cite{hartigan1981consistency}, for example. 
% : 
% \begin{equation}
% 	\hat{p} = \frac{1}{nh^d} \sum\limits_{i = 1}^n \kappa \Big(\frac{\lVert x - x_i \rVert}{h}\Big)
% \end{equation}
%where $\kappa$ is the kernel and $h$ is a bandwidth parameter. 
From the applied perspective, many state-of-the-art approaches find POIs by variants of hierarchical clustering to find groups of exemplars. This has proved useful for application-specific problems~\cite{zheng2010geolife, zhou07, zheng09} but they are largely heuristic, i.e. it is common for most clustering algorithms to have unstated or unknown statistical properties, precluding the possibility of formal inference~\cite{fraley2002model}. The framework we introduce therefore examines
{\em density-based} clustering methods as they are 
designed to infer a cluster tree~\cite{chen2016statistical}
without facing the computational hurdles of KDEs. 

A desirable property of any finite-sample density estimator is some notion of {\em consistency}.\footnote{Recall that an estimator $\hat{\Theta}_n$ whose value $\hat{\theta}$ is a point estimate of $\theta$ is consistent if, as more samples are collected ($n \to \infty$), $\hat{\Theta}_n$ {\bf converges in probability} to the true value of the parameter, i.e. $\underset{n \to \infty}{\mathrm{plim}}(\hat{\Theta}_n) = \theta$.} In 1981, Hartigan establsihed a reasonable definition~\cite{hartigan1981consistency}, often referred to as {\it Hartigan consistency}:
\begin{mydef}{\bf Hartigan Consistency}\\
Let $\mathbb{C}_{f_n}$ be the set of all high-density clusters from the cluster tree. 
For any sets $A, A' \subset \mathcal{X}$, let $A_n$ (respectively, $A_n'$) denote the smallest set of $\mathbb{C}_{f_n}$ containing $A \cap X_n$  (respectively $A' \cap X_n$). $\mathbb{C}_{f_n}$ is consistent if, whenever $A$ and $A'$ are different connected components of $\{ x : f(x) \geq \lambda \}$ (for some $\lambda > 0$), $\mathbb{P}(A_n \text{ is disjoint from } A_n') \to 1$ as $n \to \infty$.
\end{mydef}
This consistency definition essentially requires that two disjoint high-density clusters from the unknown, population density ($A$ and $A'$) will also be disjoint components in a given empirical cluster tree ($A_n$ and $A_n'$), given enough samples ($n$). 
The proposed framework for POI discovery is developed and implemented from the first computationally tractable and provably consistent algorithm that satisfies Hartigan consistency, as analyzed by Chaudhuri {\em et. al}~\cite{chaudhuri2010rates}, to be discussed in the next section. 
Having a nonparametric model satisfying this notion of consistency is important, as it transforms the unsupervised problem of POI discovery into a formal statistical estimation problem, not only enabling analysis {\it driven by data}, but requiring minimal assumptions regarding the nature of the data. 
Such a relation enables methods of formal statistical inference, allowing one to quantify uncertainty, i.e. to create hypothesis tests to discern ``true'' POIs as opposed to ``false'' POIs resulting from random noise or artifacts of low sample sizes, or to create notions of confidence in estimation~\cite{chen2016statistical}.

\subsubsection*{Consistent cluster tree estimation:}
We next motivate a recent cluster tree estimator and discuss its relationship and applicability to POI discovery for 
the propsoed framework. Recall that an empirical estimate of the cluster tree, applied over exemplars, represents a hierarchy of POIs. Viewed from this perspective, what we propose can be seen as an extension of Chaudhuri {\em et. al}'s work on the cluster tree~\cite{chaudhuri2010rates} to a trajectory mining context. 

Consider using Single-Linkage (SL) clustering, an agglomerative scheme that creates a hierarchical representation of clusters using the minimum pairwise distance $D$ between all points, as a tool for clustering exemplars. Beginning with every exemplar $x$ as a singleton, SL iteratively merges exemplars into clusters according to the {\it linkage function}: 
$$ D(x_i, x_j) = \min\limits_{x_i, x_j \in X} d(x_i, x_j) $$
SL clustering is often criticized due to its tendency to create `excessive chaining', wherein two clusters which may have been seen as generally unrelated are amalgamated by chance at a distance threshold that does not reflect the true dissimilarity between the resulting clusters. Hartigan proved SL is a consistent estimator of the cluster tree for densities in $\mathbb{R}$ (for $d = 1$) and is {\em not consistent} for any $d > 1$~\cite{hartigan1981consistency}, implying that any SL cluster that contains all the sample points in $A$ will also contain nearly all sample points in $A'$, in probability as $n \to \infty$.\footnote{The condition is related to the ``thin bridge'' between any two population modes. Fractional consistency was shown for SL if for any pair \unexpanded{$A$} and \unexpanded{$A'$}, the ratio of \unexpanded{$\inf \{ f(x) : x \in A \cup A' \}$ to $\sup \{ \inf \{ f(x) : x \in P \} : \text{paths } P \text{ from } A \text{ to } A' \}$} is sufficiently large.}
% that there exists disjoint SL clusters $A_n$ and $A'_n$ such that, in the limit, $A_n$ contains a positive fraction of the points in $A$, passing arbitrarily close to every point in $A$, and similarly for $A'$, under certain conditions.
This is reflected in the geospatial sense as well: consider the case where exemplars represent aggregated `stops' within a set of trajectories, a case that we will also consider later in Section \ref{sec:experiments_and_discussion}. If an area is observed long enough, such exemplars should naturally form an area high density in areas where people stop frequently, e.g. within buildings. In such cases, it may be useful to categorize exemplars within their respective POIs (this is done in supervised way applications extract semantic information, see ~\cite{alvares2007model} for example). However, it's also possible that there exist a few stops just outside of such buildings, which SL has a tendency to chain together. An example of this is shown in Figure \ref{fig:sl_chaining}.
\begin{figure}
		\includegraphics[width=0.34\textwidth, height=3.6cm]{sl_chaining}
		\caption{SL excessive chaining example. The bottom panel denotes a possible clustering using SL when pedestrians were found to stop between buildings. }\label{fig:sl_chaining}
\end{figure} 
This discovery motivated efforts to modify SL not only to reduce this chaining to make SL more `robust', but also to achieve (at least) Hartigan consistency for $d = 2$ and beyond. The first provably consistent estimator, which we consider in this effort, is a generalization of SL referred to as `Robust Single Linkage' (RSL)~\cite{chaudhuri2010rates}. 
%The proposed framework relies on this estimator, and thus the estimator is described in fully next. 

{\bf Robust Single Linkage:} Let $\mathcal{X}$ be a subset of $\mathbb{R}^d$. Let $\lVert \cdot \rVert$ denote the $\ell_2$ norm and let $B(x, r)$ be a closed ball of radius $r$ around the point $x$. 
The RSL algorithm is given in the listing below: 
\vbox{%
\begin{myalg}{Robust Single Linkage Algorithm}\label{alg:rsl}
\begin{enumerate}[leftmargin=*]
  \item For each $x_i$ set $r_k (x_i) = \mathrm{inf}\{ r : B(x_i, r)$ contains $k$ data points$\}$.
  \item As $r$ grows from 0 to $\infty$:
  \begin{enumerate}
    \item Construct a graph $G_r$ with nodes $\{x_i : r_k(x_i) \leq r \}$. \\
          Include edge $(x_i, x_j)$ if $\lVert x_i - x_j \rVert \leq \alpha r$
    \item Let $\mathbb{C}_{f_n}(r)$ be the connected components of $G_r$.
  \end{enumerate}
\end{enumerate}
\end{myalg}
}
The RSL algorithm has two free parameters which need to be set: $\alpha$ and $k$. SL is equivalent to RSL with the setting $\alpha = 1$, $k = 2$. 
%SL and RSL are very similar, with only a few key differences. 
Whereas SL is equivalent to (and can be efficiently computed by) the minimum spanning tree (MST) computed over all pairwise distances, RSL scales these distances by a constant factor $\alpha$, and only reduces to the MST if the components are restricted from connecting (satisfying $\{x_i : r_k(x_i) \leq r \}$) {\em within the MST computation}. Chaudhuri {\em et. al} found that RSL is Hartigan consistent and established finite-sample rates of convergence for all $1 \leq \alpha \leq 2$, with the optimal rate of convergence with the setting $\alpha \geq 2$~\cite{chaudhuri2010rates}. 

% %% Finally time to transition into the `intrinsic' definition POI
% The RSL algorithm provides a simple and consistent estimator of the cluster tree, a hierarchical representation of high-density clusters and, in this research effort, our definition of a POI. However, from the usability perspective, keeping the density threshold value $\lambda$ as a free parameter enables the existence of countless cluster configuration, to which the `best' value may not always be known or  intuitive to an analyst wishing to learn something `interesting' about the region the data was defined in. Moreover, it should be the case that any fundamental trajectory database contains an intrinsic set of POIs that can be extracted.

%%% Matt -- save this paragraph for the background or methodology section when we start talking about
%%% RSL. I think this is unrelated to the two main threads of related work mentioned above. 
%{\bf Robust Single Linkage:} In 2010, the first provably consistent algorithm for estimating the cluster tree for densities in $\mathbb{R}^d$, referred to (as above) as the Robust Single Linkage (RSL) algorithm, was published~\cite{chaudhuri2010rates}. It is not only a tractable algorithm, but it also maintains much of the elegance an simplicity of single-linkage. 
%This is significant to the clustering field: insofar as statistical learning is concerned about what a finite data sample reveals about the underlying density $f$, density-based clustering methods are concerned with finding clusters based on {\it meaningful} notions on density. This is, in essence, what many applied density-based clustering algorithms attempt to approximate~\cite{hinneburg1998efficient}~\cite{comaniciu2002mean}~\cite{kent2013debacl}. Campello {\em et al} go so far as to assert that nearly all density-based clustering algorithms are, either strictly or loosely, based on Hartigan's model~\cite{campello2015hierarchical}.
%It is perhaps not a coincidence that the popular density-based clustering algorithm DBSCAN, which has inspired numerous derivatives in both the geospatial and general clustering fields~\cite{}~\cite{}~\cite{}, has helped define the applied field of density-based clustering, was shown to coincide directly with Hartigan's notion of `rigid' clusters~\cite{campello2013density}. 


%%% -------------- Scrapped, unrefined, or redundant sentences --------------

%An natural task in geospatial analysis is to use data at hand to learn something new about the space in which the data were observed, and about the data itself. For example, if one were to cluster these spatial positions into groups, these groups (clusters) would then represent broad locations that are popular or relevant in a spatio-temporal context, subject to the constraint that {\em all} data sources reporting from the location share some amount of ``spatial and temporal similarity''. 

%See, for example, any of~\cite{kriegel2008statistical}~\cite{pavan2015finding}.  
%% Matt, is this material related to defining intrinsic points of interest? That is the focus of this section. 
%A central task in the field of trajectory data mining of concern to this paper is that of {\it knowledge discovery}~\cite{feng2016survey} from fundamental spatiotemporal databases, specifically within the geospatial context. In a recent comprehensive trajectory mining survey~\cite{zheng2015trajectory}, the entire field of trajectory mining was brought into scope, where some of the major challenges in dealing with trajectory data were discussed in detail. In the survey, trajectory mining was broken down into roughly four different categories, including uncertainty modeling (such as improving continuous interpolation approximations), pattern mining (such as the modeling of periodic patterns, location recommendation, and group behavior), classification (including segmentation techniques, activity assignments, etc.), and outlier detection.  

%% Matt - till unsure of this is related to defining intrinsic points of interest. IF this background and background
%% in the previous paragraph are connected to defining an intrinsic point of interest, then a starting
%% \subsection{Background} may be appropriate. But only if it is background necessary to understand
%% our definition or formulation of an intrinsic POI. Otherwise it is okay to chop and move to related work.
%There are application-specific motivations and methods related to the specific approaches one takes to mine trajectory data. Specifically, the type of trace activity one may be looking to model varies greatly based on domain-specific contexts. 
%%Matt - what is a trace activity? 
%As an example, consider the problem of trajectory segmentation, where the goal is to 'segment' a trajectory into different segments as a means of enabling a different type of knowledge discovery, sometimes referred to as {\it subtrajectory mining}~\cite{zheng2015trajectory}. Trajectory segmentation might be based on a time interval, or based on relative changes in the shape of a trajectory, or on some semantic meaning such as velocity. Another difficult challenge is the fundamental problem of modeling sampling rate, where the goal is to reduce and understand the inherent uncertainty that exists when trying to approximate the continuous trace or ``path'' an object took from a finite set of discrete points. 
%Intuitively,  
% ``it is intractable to define a similarity metric for comparing trajectories...since trajectories are probably generated with different sampling strategies or at different sampling rates''~\cite{feng2016survey}.
% Several other examples of approaches to general trajectory mining are given in the related works section \ref{}.
%
%In short, the field of trajectory mining is both large and diverse, and the approaches taken to mine trajectory data vary based largely on the context and the domain in which the approach was developed, all of which are valid, with varying degrees usability. However, this fundamentally leaves the question unanswered as to whether there can exist a generalizable POI discovery method for geospatial data, applicable to {\em any} trajectory database. 
%For the purposes of this paper, any of the approaches to trajectory mining proposed are compatible with the framework proposed. 

% Matt, now we are talking!!  
%\subsection{Intrinsic Point of Interests for Trajectory Databases}
%If the observation window of a particular object coincides both spatially and temporally with the observation window of another object, it seems intuitive that these objects might be related. Thus, it is desirable to create some structured means of using the information available from an object's 'movement' through a common space to learn something interesting about the space itself. It is from this key intuition that we posit that an {\em intrinsic point of interest} be defined as a geographical region {\it defined by the data, i.e., track locations over time} that exhibit significant a high a degree of {\bf spatiotemporal density} (we defer to give a more rigorous definition below).
%
%
%Spatiotemporal similarity immediately suggests that some kind of clustering method be used to unearth
%intrinsic POIs. 
%%Matt, need to elaborate. 

%% Matt- here is a paragraph to get into density based clustering. 
%%

%To illustrate this problem more clearly, consider a subset of points (positions) gathered from noisy trace data, initially collected from an Aerial Surveillance platform. This data, after projecting the movement data onto a roadmap from Google Maps, is illustrated in \ref{fig1}. Although commonly used for formal density estimation and discriminant analysis, It becomes immediately clear that {\it model-based} approaches such as the well-known Gaussian Mixture Modeling (GMM) are inapplicable to describe trace data directly due to the known tendency for GMMs to produce clusters of hyper-elliptical or hyper-spherical shapes. Furthermore, parametric approaches to mixture modeling explicitly require assumptions to be how the underlying processes that produced  
%
%that attempt to describe the underlying density of the trace data directly are seemingly inapplicable.  to the situation where data 
% \begin{figure*}
% \begin{multicols}{2}
% 	\includegraphics[width=0.5\textwidth, height=5cm]{intersection_points}\label{fig1}
%     \caption{Subset of movement data recorded over an intersection.}
%     \includegraphics[width=0.5\textwidth, height=5cm]{intersection_kde}
%     \caption{Kernel Density Estimate using gaussian kernel estimator. }\label{fig2}
% \end{multicols}
% \end{figure*}
% 

%% The aside is not relevant to the topic of the subsubsection, POI discovery. 
%Although the association with Hartigan was not made, it's worth noting that the use of kernel density estimators or density `influence' functions to create a hierarchy of clusters defined as the maximally connected, upper-level sets of the estimated density was also explored by  Hineburg {\em et. al}~\cite{hinneburg2003general}, although consistency was not shown. 

% This idea of an `unknown' stops  
%% ------------
%% need to look like? What would the building blocks be (e.g. the notion of shapes \in R^d as you mentioned above).

% There are perhaps innumerable techniques to define what a `naturally occurring' cluster is.  There is no standard definition of a ``point of interest.'' There are perhaps innumerable mathematical procedures that assign value to how 'interesting' a region of the data space is. From the perspective of detecting interesting locations within the subdomain of movement data alone, a number of questions often arise: How does one formally define a 'location'? What are the properties that describe how 'interesting' a location is i.e. what are the attributes that quantify this notion of 'interesting'? If these attributes can be readily decided on, can the modeling of points of interest be recast as statistical model choice problem, allowing the possibility of formal inference?
 
 % These are difficult problems that have been addressed over and over in a variety of contexts[space-time paper]. 
 % List of papers doing POI discovery, potential list of applications and their definition of a point of interest. 
%A POI is a region of the geospace that is often visited and, depending on the intention of the model, exhibits some features that are inherently 'interesting;' examples might include places such as restaurants, places of cultural significance,   It seems intuitive that perhaps one of the primary reasons it is difficult to formally define exactly what a ``Point of Interest'' is is due not only the obvious subjectivity involved with quantitatively defining how ``interesting'' something is, but also in the specific methodology in which one determines the relations between POIs.   
% 
% Such groups cannot effectively be captured using a parametric, model-based approach. There are many situations where data are constrained to be observed in arbitrarily shapes due to environmental influences. This creates "natural groups" often exhibit non-convex, arbitrarily shaped forms that in the context of human supervision, can be easily and unanimously distinguished. Despite the effectiveness of density-based approaches, many are inherently heuristic by design, preventing the capability of formal statistical inference.
 


==> ClusterTree POIs/introduction.tex <==
The development and deployment of location acquisition systems have enabled large scale capturing of `movement' or `trajectory' data from people, cars, and other objects. Technologies like global positioning systems (GPS), global system for mobile communications (GSM), wide area motion imagery (WAMI), and radio-frequency identification (RFID) allow organizations and governments to collect and exploit trajectory patterns in many scenarios.
%% 
More recent initiatives (e.g. Uber's Movement\footnote{\url{https://movement.uber.com/cities}} and IBM's Smarter Cities\footnote{\url{https://www.ibm.com/smarterplanet/us/en/smarter_cities/overview/}} programs) have even made such data available to the either the public or city planning experts at large. 
With the rise in importance of this data comes prevalent use of Geographic Information Systems (GIS) and related platforms such as ArcGIS\footnote{\url{https://www.arcgis.com/}} and Mapbox\footnote{\url{https://www.mapbox.com/}}. Other related use cases of GIS information have also emerged for surveillance~\cite{chang2009combining} and location-based service (LBS) applications~\cite{virrantaus2001developing}. In many of these applications, trajectory data is exploited for knowledge acquisition tasks~\cite{gonzalez2008understanding}, the integration of movement patterns to uncover ``patterns of life" over a region~\cite{zheng2010geolife}, to expand situational awareness in crises~\cite{zhang2017emergency}, and to support the value added by a LBS application~\cite{figueiredo2016tribeflow}.

In many of these knowledge acquisition tasks, the notion of a ``location" or ``point of interest" (POI) is foundational to understanding the entirety of the common space in which the data are observed~\cite{pavan2015finding}. For example, mapping systems must know the position and geometry of locations for navigation and automated guidance control purposes. In LBS applications, the POIs and metadata such as their popularity (e.g. `star-rating') are necessary to provide useful location recommendations~\cite{zheng09,park2007location, figueiredo2016tribeflow}. 
Because POIs are not available from `raw' trajectory data captured by location acquisition systems, they are often {\em extrinsically} defined by gazetteers such as Google Places, FourSquare, GeoNames, or OpenStreetMap. 	%% Matt, I love the word extrinsic.
Yet external sources of location data present many difficulties when faced with the problem of understanding how a given trajectory dataset relates to the underlying geographical area where it was observed. For example, many gazetteers store varying types of either POI metadata or POI relational data, allowing gazetteer-derived information to present a source of {\em bias}. Furthermore, relying on gazetteers explicitly {\em defines} the set of POIs that exist in a given geographical region. When there  is disagreement on this definition, analysis becomes difficult. Furthermore, with POIs defined {\it a priori}, one is faced with the problem of ``fitting'' observed trajectory data to models defined by such POIs, many of which may or may not be relevant to the given data at hand. For example, it may be desirable for a city-planner gathering movement (trajectory) data following a public event to discover `bottleneck' congestion areas like parking lots, roads, or sidewalk segments for the purpose of traffic analysis. In this situation, it would more useful to discover POIs directly {\em from the data itself} during the event, but such geographical POIs may not be available in a gazetteer. 

To over come these challenges, this paper investigates the POI discovery problem in the most generic context possible. We ask: {\em given only trajectory data, without access to gazetteers, can we infer subregions within a geospace that are ``interesting" enough to call it a POI?}
We seek {\em intrinsic} POIs, which are POIs recoverable without the use of a gazetteer, are completely defined by observed movement patterns, and can be used for any domain-specific application and at any scale (e.g. from movements within a building to movements across an entire city region). 
To make such a definition meaningful, we build off recent theoretical work in density-based clustering and introduce a data-driven, statistically rigorous definition of a POI applicable to trajectory data of any (and even mixed) resolution. The definition follows from a recent minimax analysis of the consistency of hierarchical density superlevel set estimators. We use this definition to present a {\bf parameter-free} framework for extracting intrinsic POIs, i.e. yields an optimal unsupervised 
solution without ad hoc parameter-tuning.\footnote{We see this as a necessary form of {\bf usability}, an important feature to have in the modern clustering era. It is well-known that having several sensitive, real-valued parameters results in combinatorial explosion of the parameter space of an algorithm, resulting in the need for the user to use one or more parameter-tuning methods to arrive at a solution that befits the application.}
A comparative analysis is performed on realistic simulations involving both vehicle and pedestrian traffic. Validation results show marked improvements in fidelity against several state of the art (SOTA) algorithms. Of interest to the authors, the simulation settings, the resulting traffic data, the validation code, and the framework itself is all {\bf completely reproducible} and {\bf open source}, available online.\footnote{<Anonymized for review purposes.>}
%The remainder of the paper is organized as follows. In Section \ref{sec:methodology}, we introduce definitions and the proposed framework for intrinsic POI discovery. In Section \ref{sec:experiments_and_discussion}, we demonstrate a use case for the framework using urban traffic data, and present a comparative analysis using several SOTA clustering methods. In Section \ref{sec:related_research} we discuss related work. Finally, Section \ref{sec:concluding_remarks} summarizes the contributions of the paper, and concludes with remarks on future work that could further extend the framework.


%% ================= FROM DETACHED HEAD =========================

%A given POI discovery method only carries merit if the data collected and a system's definition of an `interesting location' matches with the notion of a POI the method encodes. For example, many LBS approaches will give travel recommendations using locations known {\it a priori} through preexisting gazetteers, such Google Places, FourSquare Venues, OpenStreetMap POIs, etc., which we will refer to generally as {\it knowledges bases}. 
%The applicability of such methods to observed data sets are categorically dependent on the degree to which such knowledge bases align with the intent of the analysis, and whether the data itself reflects align with such knowledge bases. 
%%Matt, not sure I understand. Note that the first example was very applied and specific, the second example is vague. 
%For example, having knowledge of the popularity of every restaurant within a city may be useful for food-service recommendation applications, but such knowledge may prove useless to applications which depend on the locations {\it not} known by the knowledge base. Consider the scenario where a city-planner has gathered data over a given time period recording samples of traffic density after a public event such as concert or festival and would like to analyze the impact of the event on traffic congestion in that area for the purpose of future event planning. In this type of analysis, the focus of the analysis is {\it data-driven}
%This has known implications in the field of urban design and transportation planning, where the relationship between ``the built environment'' and travel behavior is inherently linked to the complex structure of the geographical environment and the distribution of activities across the space~\cite{handy2002built}. 
%This systematic assumption that having known data corresponding to the conventional interpretation of a `location' (such as a building or a park) renders such knowledge base reliant models, which we will refer to as {\it gazeteer-driven} models, unusable in geographical areas where such data is not available, incomplete, or biased.

%% Provide some motivating concepts behind the idea of an intrinsic POI
%% Matt, unsure what the purpose of this paragraph is. The previous paragraph was about why narrow POI methods
%% are not suitable and the need for a more general approach. So this paragraph should be about the general approach
%% or defining this general approach. 
%For all of the reasons stated above, models built existing knowledge bases are inherently  The question remains POI discovery may be thought of as {\it trajectory pattern mining}. The conceptual model underlying many trajectory mining approaches is that objects may exhibit similar spatiotemporal patterns either individually or en large, and that these patterns carry valuable information about the common space in which they were defined. For example, if the estimated speed of multiple trajectories corresponding to vehicular traffic sharply decreases and the vehicles are close in both space and time, it's intuitive to deduce that they may be stopped at a traffic light, or congested in a traffic jam. Methodologies that rely on the spatiotemporal components of either individual or groups of trajectories (with or without external geographical information) to define locations will be referred to as {\it data-driven} approaches.

%% Related intrinsic POI approaches (sort of) 
%% Matt, unsure where classic ML approaches come from here. I think this and the previous paragraph should be merged 
%% and focused in. Maybe it is about a class of 'more general' methods for POI discovery. Still, the disadvantage is that 
%% the meaning of a POI is not agreed upon, so each of the general methods are discovering quite different things. 
%However, as with many patterns in spatiotemporal data mining, these patterns are merely discrete observations of a continuous space, break assumptions of independence due to high autocorrelation, and often manifest in localized rather than globalized contexts, rendering the use of classical machine learning approaches unsuitable~\cite{shekhar2015spatiotemporal}. 
%Perhaps as a direct result, the trajectory mining field has been largely progressed by ``extensive and intensive'' individual efforts~\cite{zheng2015trajectory}. 
%Nonetheless, conceptual models have been proposed for dealing with trajectory data; one such model postulates that trajectories, and the subsequent spatiotemporal patterns extracted from them, are essentially driven by the semantics the application associates with trajectory itself~\cite{parent2006conceptual}~\cite{spaccapietra2008conceptual}. Popular extensions to this conceptual model include the ``Stops and Moves of Trajectories'' (SMoT) family of classification algorithms~\cite{alvares2007model}~\cite{palma08}~\cite{rocha2010db}, where the premise of the analysis is that by partitioning trajectory data into a labeled set of `stop' and `move' segments, one can take then annotate these segments with semantic information, derive specific mobility patterns, and as a result {\it discover} `interesting' locations. In particular, Alvares et. al generalizes the concept of a location as a pre-existing, topologically-closed polygon within a common space in which the observed trajectories are defined. The SMoT algorithm, fundamentally built on heuristics, then delineates between segments types by detecting when a sequence of points within a trajectory intersected with these known geometries, thereby `enriching' the trajectory data with semantic information. Palma et. al extended this concept~\cite{alvares2007model} by classifying stops that occurred within such known polygons as `known stops', whereas stops found outside of these shapes were classified as `unknown stops', of which the latter are determined through a clustering approach. 
%
%Indeed, Spaccapietra et. al anticipated a number of conceptual and practical key ideas that have also been used by many modern trajectory mining approaches. Zheng et. al pioneered the use of `stay points', corresponding to an aggregation of consecutive GPS points that collectively are within a given time and distance threshold supplied by the user, characterizing a `virtual' location~\cite{zheng09}. Zhou et. al consider the use of their `DJ-clustering' algorithm~\cite{zhou2007discovering}, a derivative of the well known DBSCAN algorithm~\cite{ester1996density}, as a means density-based approach to determining ``personally meaningful'' locations. One need not look far for additional extensions of this idea; consider any of the following: ~\cite{}~\cite{}~\cite{}~\cite{}~\cite{}~\cite{}.  

%%% Everybody uses density, nobody has consistency
%% {\bf Deficiencies of current approaches:}
%%% Matt-- I think this is how we lead a paragraph that follows one talking about the varying definition of a point of interest
%As the definition of {\em what a point of interest is} varies widely, often relying on application-specific information or  algorithmically defined heuristics, so too do the meanings behind any attempt at inference that ensues. This begs the question:
%{\bf it is possible to define a notion of an {\em intrinsic} POI?} By {\em intrinsic}, we mean a point of interest that is present even without the availability of domain-specific information, and it thus completely defined by the most basic elements of a trajectory database, namely an object and its spatial and temporal observations. 
%%% Matt, in general, use POI everywhere or point of interest everywhere. Use the other one nowhere. 
%We seek a {\bf rigorous} definition of an intrinsic point of interest that is determined by trajectory {\it exemplar positions}, as well as a tractable framework to extract such POIs that does not necessarily {\it depend} on domain-specific external knowledge, but can nonetheless be enhanced by it. 
%%% Matt, I don't quite understand the above sentence. It may be loaded with two different ideas, that are related (supplement)?
%%Matt, the definition is rigorous, not the approach. I thus don't know what it means for a definition to promise confidence 
%% measures, enables statistical inference, etc. But I like the criteria you are using for `rigorous'. 
%By rigorous, we mean a definition that has a precise mathematical expression rooted in formal probability theory, thus enabling future promises of confidence measures, statistical inference, and has any prerequisite assumptions regarding the data stated or known a priori.
%%% Matt, we are doing a framework, not an algorithm. Something to note for the rest of the paper. An alg may be a component
%%% of the framework
%From this interpretation, developing a rigorous definition of a POI and a framework capable of discovering them is challenging; location discovery is fundamentally an unsupervised problem, and in the context of data clustering (the most fundamental unsupervised learning setting) it is well known that no domain-independent approach or validation measure has been proven to produce a 'best' result in both real and synthetic scenarios~\cite{kleinberg2002impossibility, gurrutxaga2011towards, guyon2009clustering, von2012clustering}. 
%%% Matt, why is conformance to the MAU problem a bad thing? Just elaborate briefly. 
%Worse yet, in practice, geographical locations tend be hierarchical in nature, resulting in any analysis performed being subjected to the well-known {\it Modifiable Areal Unit Problem} (MAUP)~\cite{wong2009modifiable}. MAUP is an intuitively difficult form of statistical bias in the specific context of geographical analysis that results from the aggregation of data areal units that are unrepresentative of the underlying data. 
%
%%% This paragraph is great. 
%There are nonetheless many commonalities between the existing approaches that could support a definition of an intrinsic point of interest. For example, many of the proposed location discovery approaches augment existing clustering algorithms~\cite{}~\cite{}~\cite{}~\cite{}~\cite{}, motivating a theoretical exposition of the statistical nature of clustering. Of these approaches, nearly all of them rely on {\it density-based} methods, perhaps due to their applicability to capturing so-called `natural clusters', or clusters that generally follow non-convex shapes, which inevitably appear in the geospatial settings. 
%Another benefit of density-based methods is the tendency for such approaches to identify localized patterns, usually with respect to some user-supplied scaling parameter. 
%For example, a subregion that exhibits a high density of track positions during rush hour (e.g an intersection) may be an ``interesting" location for a system doing traffic congestion analysis, and is `localized' in the sense that the traffic demand was sufficiently high in the region, but much of the surrounded space exhibited a relatively lower traffic density, where these density levels correspond to threshold values the user considers applicable to the domain of interest. 
%In the effort the follows, we examine the relationship between these localized movement patterns and nonparametric, hierarchical, density-based methods in a geographical setting.

%% Matt, parameter-free, flexibility, reproducibility are not contributions. Rather, they are properties of your contribution (the method and the validation). I think we can save space and make this all flow a bit more by making this itemize a paragraph. 
%{\bf Contributions}. Building off recent theoretical work in density-based clustering, this paper contributes the following: 
%\begin{itemize}[leftmargin=*]
%	%% matt, density estimates of what? 
%	%% - of i.i.d samples of any distribution in R^d 
%	\item {\bf Rigorous Definition of a POI:} 
%	We propose a statistically rigorous, multi-resolution definition of an intrinsic POI. The definition follows from a recent minimax analysis of the consistency of nearest-neighbor density estimates that form {\it high-density clusters}, where a high-density cluster is a maximally connected upper level sets of the form $\{x : f(x) \geq \lambda \}$. The hierarchical representation of this concept, known by many as the {\it cluster tree}, has a long history of analysis associated with it (see \ref{sec:motivation} for more details on this). Unlike {\it many} existing approaches, the unsupervised version of approach is {\bf parameter-free} in the sense that our approach has one free (integer) parameter that acts as a fairly smoothing factor\footnote{We see this as a necessary form of {\bf usability}, an important feature to have in the modern clustering era. It is well-known that having several sensitive, real-valued parameters results in combinatorial explosion of the parameter space of an algorithm, resulting in the need for the user to use one or more parameter-tuning methods to arrive at a solution that befits the application.}. Additionally, we discuss how one can incorporate domain-specific knowledge in the form of instance-level constraints about particular geospatial features of interest as a means of semi-supervised POI discovery, enabling the framework to be {\bf configurable} for specific applications. All of the source code, validation tests, and data mentioned in this effort is available publicly online\footnote{Hosted at: \url{https://github.com/peekxc}}. % TODO 
%	\item {\bf Validated Results} 
%	We demonstrate the generalizability of the approach with evaluations over both synthetic and real geospatial data taken from a wide variety of contexts. The framework itself is {\bf open-source}, publicly available at \url{link-to-source}. Furthermore, the results are fully {\bf reproducible}, with the synthetic data sets and tests used for validation also available at the given url.  
%\end{itemize}	
%
%The remainder of the paper is organized as follows. In Section \ref{sec:motivation}, we introduce the problem to be solved and examine some of the preliminary motivation and notation that the current literature uses. In Section \ref{sec:related_research} we discuss related work and, in particular, highlight the relationship between many efforts and the work presented here. In Section \ref{sec:proposed_framework}, we introduce our framework for nonparametric POI discovery. In Section \ref{sec:experiments_and_discussion}, we demonstrate use cases for our framework with both synthetic and real geospatial data and present a comparative analysis using several SOTA clustering methods and demonstrate the applicability of our methodology to geospatial-centric analysis's. Finally, in Section \ref{sec:concluding_remarks} we summarize the main contributions of the paper, and conclude with a few remarks on future work that could further extend the framework.  
% 
 
 
 
 
%%% -------------- Scrapped, unrefined, or redundant sentences --------------
%% Everybody uses density, nobody has consistency
% {\bf Deficiencies of current approaches:}
%% Matt-- I think this is how we lead a paragraph that follows one talking about the varying definition of a point of interest
%% Matt, in general, use POI everywhere or point of interest everywhere. Use the other one nowhere. 


% Collective groups of objects that move along similarly dense paths at multiple `snapshots' of time (sometimes referred to as convoys) allow the discovery of knowledge related to the evolution of such groups of objects~\cite{kalnis05}, with a common example being the study of migration patterns of various breeds of birds. 
% Many claim that domain-independent clustering is essentially the task of density estimation~\cite[]. ``..In so far as clustering is domain independent, it is about estimating probability distributions or functionals of them. If that is accepted, then it can be easily formalized using loss functions.''~\cite{guyon2009clustering} 
% The final recommendation of Luxburg et. al given regarding how to make a real impact in an application area of clustering is stated in the conclusion section: ``What is missing is not ``better'' clustering algorithms but a problem-centric perspective in order to devise meaningful evaluation procedures.''~\cite{von2012clustering}. 
 %Intuitively, the inductive bias adopted by the clustering model is conceptually equivalent to the choice of a loss function from the field of supervised classification. However, unlike supervised learning, it's not always readily evident what loss function (or validation measure, see~\cite{gurrutxaga2011towards}) to use. 
% \begin{figure*}
% \begin{multicols}{2}
% 	\includegraphics[width=0.5\textwidth, height=5cm]{intersection_points}\label{fig3}
%     \caption{Observed trajectory data over a popular intersection at the Ohio State University.}
%     \includegraphics[width=0.5\textwidth, height=5cm]{intersection_kde}
%     \caption{Bivariate Gaussian Kernel Density Estimate (KDE) of trajectory data using manually set 
%     bandwidth selection. }\label{fig4}
% \end{multicols}
% \end{figure*}


% It would thus be ideal to have a model that, given no prior information but the geospatial data itself, can discover 'interesting' locations making minimal assumptions on the data, but is adaptable to incorporate such metadata in a reasonable way. 
%We assert that an `intrinsic' POI is a random variable defined over the space of spatiotemporal density representing similar mobility patterns.  
%We assert {\bf yes}, there must 
%be a way to define rigorously the notion of an intrinsic point of interest in a trajectory database. 
%Matt, why do we assert yes? 
%Being able to identify such intrinsic points of interest would be useful in a variety of contexts. For example, it
%is a common exercise to define some measure as a means of modeling the geographical influence of locations within a city~\cite{}, the traffic changes caused by planned changes to a road network~\cite{}, for the purposes urban planning efforts~\cite{}, or for route recommendation systems~\cite{}.
% Not sure if I should go into 'intrinsic' essentially meaning high-density modes 
% Matt, I think that detail is too fine. We also need to bump up motivation for why anyone would be interested in an intrinsic POI. 

% TODO: relate the commonalities of different approaches to density-based clustering 
%Finding intrinsic points of interest appears to be difficult since even the notion of an {\em intrinsic} point of
%interest is not well defined. Towards establishing this definition, we observe that many research efforts in the domain of POI discovery share a common way to define a `location': they first leave some discretization of the space as a parameter to user, and then turn to a clustering algorithm that defines a point of interest by a high ``density" of observations within discrete geospatial areas. This discretization is often done by many users, with discrete regions defined by locations scrapped from existing crowdsourced knowledge bases (e.g. Google Places or Foursquare).
%
%
%In other situations, such as efforts within the domain of LBS applications, having metadata corresponding to the popularity of known locations may be considered more relevant to determine if a location is ``interesting"~\cite{}. Moreover, many POI discovery techniques require very specific metadata about a geospace, such as the preferences of a track~\cite{}, information about geometries of the existing locations or venues in the geospace~\cite{alvares2007model}, latent variables inferred from a friendship network~\cite{}, or a history of past locations that a track may have visited~\cite{zheng09}. For example, in LBS recommendation applications, Collaborative Filtering (CF) techniques have proved extremely useful for the purpose of location recommendation, wherein the general idea is to associate metadata or 'tags' with either locations known {\it a priori} or with locations discovered from the data to make user-specific recommendations~\cite{}~\cite{}. 
%Such tags and location annotations in the data define a discretization of the geospace. In another example,
%location-based Social Networks (LBSN) methods have also become massively popular for modeling user preferences for the purposes of locations recommendation~\cite{}...
%%%Matt, how does LBSN match the common way of defining a location that you discuss?   
%%A general metholdogoy that has appeared in the world of POI discovery and recommendation appears to be of the form: 
%$$\text{Sequential Pattern Mining} \to \text{Clustering} \to \text{Social Network}$$    
%Of the latter approaches, many then take a density-based clustering method to group observations
%around points of interest due to their ability to capture so-called ``natural'' clusters. 
%%%Matt, I don't understand the sentence below. Need something clear to explain why density-based clustering
%%% feels like a good way to go for geospatial data (if I am inferring the right thing from your writing).
%Intuitively, this seems to corresponds more readily to the geospatial context especially. Consider a geospace defined over a road network, where tracks are observed moving throughout a road network over time. In an urban environment, the structure of the roads and the surrounding landscape will cause the trajectory data to manifest in shapes matching the movement patterns of the network, which can then be of any arbitrary shape. 
%While the use of density-based clustering over observations seems like a natural way to define a
%point of interest, we do not consider any present method to define {\em intrinsic} points of interest. 
%This is because present methods require a predefined separation of a geospace into 
%discrete regions, each of which is a ``candidate" to be a point of interest. Relying on this external information
%goes against the idea of an intrinsic point of interest because the possible points are limited by
%the information provided from this external source. Instead, an intrinsic point of interest must be one
%that only requires the minimum information present in any trajectory database. 

%% Matt - the exposition below is good and appropriate. However, we need to tie this all back to the main idea of this paragraph. We started by casting doubt on our work -- it seems like finding intrinsic POIs are impossible. We have to end the paragraph with reason to be hopeful, perhaps based on past work or discovers in the analogous problem of data clustering -- or we need to lead off this paragraph in a different way, that still ties itself to the discussion in the previous paragraph. 


%% Matt - I took your old paragraph and try to merge here to organize and melt the ideas together. 
%% Note that the main idea of this paragraph has to be that we want to find a rigorous definitino of a POI and
%% a framework to extract it. So this paragraph needs to support how we are going to find these things. 
%% leave the reader hopeful that we have a solution and give her some intuition behind what we'll do. 
%% I'm not sure yet if the sentences in this paragraph and the cites fit this idea. If not, maybe they belong
%% in section 2. 



==> ClusterTree POIs/methodology.tex <==
 \subsection{Finding intrinsic points of interest}
Using a consistent cluster tree estimator, such as RSL, on a set of exemplars creates a hierarchical representation of POIs. However, a nested set of multiple solutions is not always desirable, and a `flat' solution (where each point is assigned a single label) may be preferred. A traditional approach in hierarchical clustering, ``cutting'' the empirical cluster tree at a given density threshold value $\lambda$ yields a set of high-density clusters
$\mathbb{C}_{f_n}(\lambda) = \{C_1, C_2, \dots C_m\}$
that form $m$ POIs, a possible `flat' solution. 
However, the choice of $\lambda$ forces all POIs to be of the same scale, requires the user to know which  granularity to choose {\em a priori}, affecting the size and kinds of POIs discovered. For example, a small $\lambda$ may define shops in a mall as POIs, while a larger $\lambda$ may define the mall itself as a POI. It may not be known ahead of time what granularity level is relevant. 
Furthermore, it is reasonable to expect that relevant POIs exist at multiple levels of granularity, such that a sprawling city park and a small restaurant could both constitute a POI. 
Thus, it would useful to have some sensible notion of ``cluster quality'' that can be used (and optimized) as an objective function to discover POIs that are not dependent on the analyst's choice of $\lambda$, and are {\em strongly intrinsic to the geospace itself}, e.g. are {\bf intrinsic POIs}. 

To capture POIs of any scale and hence satisfy our notion of an intrinsic POIs, we first recall that high-density clusters are contiguous, relatively dense areas of the data space, separated by contiguous and relatively non-dense areas, defined over a working definition of density over a set of exemplars. From a statistical point of view, we can think of a high-density cluster as a set of points with high density around some ``neighborhood'' or volume of the support. M{\"u}ller {\em et. al} quantify this using a functional called {\em excess of mass}~\cite{muller1991excess}: 
\begin{mydef}  {\bf Excess of Mass}\\
For a $C_i \in \mathbb{C}_{f_n}(\lambda)$ for some value of $\lambda > 0$, the {\bf excess of mass} of $C_i$ is given by: 
	\begin{equation}\label{eq:4}
		E(C_i) = \int_{x \in C_i} \Big( f(x) - \lambda_{min}(C_i) \Big)\text{ }dx
	\end{equation}
\end{mydef}
where $\lambda_{min}(C_i)$ represents the lowest density level $C_i$appears.
Initially, this measure seems like a reasonable definition of the ``quality" of a clustering within the cluster tree estimate. Considering the definition of a high-density cluster from Equation \ref{eq:poi}, where a cluster exists along a mode of local maximum of the underlying density, it's far too likely that a finite-sample estimation may empirically find a mode at a given point $x_0$ if the data is sparse, allowing an arbitrarily low probability associated $x_0$ to be classified. A more interesting result would be to associate a high-density cluster with a region that exhibits relatively high probability {\em over a  neighborhood}. See M{\"u}ller {\em et. al} for visualization, along with a more in depth description of this functional~\cite{muller1991excess}. 
%%Why? 
However, as Campello {\it et. al} remark, this measure exhibits monotonic behavior in any direction varying the density-level $\lambda$ in the hierarchy, and instead propose an alternative, {\em local measure} of cluster quality~\cite{campello2015hierarchical}:
\begin{mydef}  {\bf Relative Excess of Mass}\\
For a $C_i \in \mathbb{C}_{f_n}(\lambda)$ for some value of $\lambda > 0$, the {\bf relative excess of mass} of $C_i$ is given by: 
	\begin{equation}\label{eq:4}
		E_R(C_i) = \int_{x \in C_i} \Big( \lambda_{max}(x, C_i) - \lambda_{min}(C_i) \Big)\text{ }dx
	\end{equation}
\end{mydef}
%% Matt check this..
where $\lambda_{max}(x, C_i) = \min\{ f(x), \lambda_{max}(C_i)\}$ is the density level beyond which $x$ is no longer part of $C_i$, and $\lambda_{max}(C_i)$ is the highest density beyond which $C_i$ either becomes disconnected (creating separate components) or disappears (creating singleton clusters). It is important to note that relative excess of mass is defined in terms of $\lambda$ values associated with a specific {\em cluster}, as opposed to a specific {\em clustering}. 
This implies that an `optimal' clustering with respect to the relative excess of mass estimate may not occur at a fixed,  {\em global} density threshold, but rather as a result of several {\em local} density thresholds applied to the hierarchy. Intuitively, if a given cluster $C_i$ contains many points that have high density relative to $\lambda_{min}(C_i)$, such a cluster will exist across several thresholds of $\lambda$ and is thus robust to fluctuations in the scale of analysis. For this reason, the relative excess of mass can be thought of as a measure of cluster `stability' across different density levels, which we posit reflects an {\em intrinsic} POI that is innately defined by the dataset independent of density level. Such intrinsic POIs are thus defined as follows: let $\delta_i$ be an indicator equal to 1 if cluster $C_i \in \mathbb{C}_{f_n}$ represents an intrinsic POI and 0 otherwise. Assign values to these indicators such that the following is maximized: 
 \vspace*{-0.085cm}
 \begin{equation}\label{eq:10}
 	\begin{aligned}
 		& \underset{\delta_1, \dots, \delta_m}{\text{maximize}}
 		& & J = \sum\limits_{i = 2}^m \delta_i E_R(C_i) \\
 		& \text{subject to}
 		& & 
 		\begin{cases} \delta_i \in \{ 0, 1 \}, i \in \{2, \dots, m\} \\
 		\text{exactly one }\delta(\cdot) = 1 \text{ per disjoint branch}
 		\end{cases}
 		\end{aligned}
 \end{equation}
 %% Matt, we need to dig a bit into this optimization. No long details, but a few sentences or key points
 %% how how this can be solved. 
 Where the ``per disjoint branch'' constraint means that the indicator function $\delta(\cdot)$ equals 1 exactly once for all clusters in each path from a leaf node to the root of the cluster tree. The optimization of this objective function is beyond the scope of this paper; we refer to Campello {\em et. al}'s cluster extraction method for general cluster hierarchies~\cite{campello2013framework} to solve this optimization, as it was developed alongside an estimator very similar to RSL, is capable of producing an optimal result at several density levels, and accounts for the density thresholds at which points become noise (fall along densities below a given threshold). 

==> ClusterTree POIs/relatedwork.tex <==
The trajectory field has been largely progressed by ``extensive and intensive individual efforts''~\cite{zheng2015trajectory}. Nonetheless, conceptual models have been proposed for how to deal with the patterns within trajectories and how to relate such patterns to geographical areas of interest for various purposes. One such model postulates that trajectories and their spatiotemporal patterns are essentially driven by the semantics the application associates with trajectory itself~\cite{parent2006conceptual}~\cite{spaccapietra2008conceptual}, and have contributed significantly to the ``Stops and Moves of Trajectories'' (SMoT) family of classification algorithms~\cite{alvares2007model, palma08, rocha2010db}, where the premise of the analysis is that by partitioning trajectory data into a labeled set of `stop' and `move' segments, one can take then annotate these segments with semantic information, derive specific mobility patterns, and as a result {\it discover} `interesting' locations. 
Alvares {\em et al.} developed IB-SMoT to find interesting positions based on semantic annotations describing the places a trajectory visited~\cite{alvares2007model}. Palma {\em et al.} reduced IB-SMoT's reliance on prior knowledge about positions that are likely to be interesting by incorporating the speed at which tracks are traveling with their variation CB-SMoT~\cite{palma08}. DB-SMoT finds clusters of common trajectories based on similar direction changes and stopping points~\cite{rocha2010db}. Zhou {\em et al.} tackle the problem of finding positions of interest to an individual track based on data about a track's location preferences, position over time, and tags of locations provided by web services such as Google Maps~\cite{zhou07}. 

Many related efforts encode or are reliant on varying notions of an ``interesting place'' using, for example, techniques from natural language processing (NLP)~\cite{gabrielli2014tweets}, data clustering~\cite{rocha2010db, zhou07, uddin2011finding}, sequential pattern mining~\cite{xiao2014inferring}, and social network analysis~\cite{zheng2011location} methods. Zheng {\em et. al} pioneered the use of `stay points', corresponding to an aggregation of consecutive GPS points that collectively are within a user-supplied time and distance threshold, thereby characterizing a `virtual' location~\cite{zheng09, zheng2010geolife}. It is interesting to note that Zheng {\em et. al} used OPTICS to create a hierarchical clustering `stay points' for an LBS-type application with Microsoft called `Geolife'~\cite{zheng2010geolife}. Indeed, Zheng anticipated a number of developments in the trajectory mining field~\cite{zheng2015trajectory}; the theoretical cluster tree may be viewed as a more statistically based conception of the`Tree Based Hierarchical Graph' that is used to represent POIs in that application as well. 

It's worth noting that our definition of an intrinsic POI, having a more theoretical foundation in density-based clustering, is both conceptually very similar to OPTICS and computationally, more recently, to Hierarchical DBSCAN (HDBSCAN)~\cite{campello2013density}. There exist a number of commonalities between both OPTICS and DBSCAN and the theory of the cluster tree. A comprehensive exposition of this relationship is beyond the scope of this paper, see Campello {\it et. al}~\cite{campello2015hierarchical} for a thorough review of the subject. Although it's not mentioned in such efforts, the usage of RSL with a relative excess of mass functional to cluster extraction is equivalent to the flat clusters ``HDBSCAN'' extracts with a setting of $\alpha = 1$ and $k = \mathit{minPts}$. However, the asymptotic consistency of the setting of the pair $(\alpha = 1, k \sim d \log n)$ has not been established~\cite{chaudhuri2010rates}. When $alpha = 1$, $k$ must be much larger, exponential in the dimensionality of the data set, $d$. Thus, we use RSL with $\alpha \geq \sqrt{2}$. 

==> ClusterTree POIs/results.tex <==
We next evaluate the proposed framework for intrinsic POI discovery. Because intrinsic POIs do not rely on gazetteers and may manifest themselves in unknown locations, evaluation on real data validated against ``ground truth" external knowledge (such as imported location data from sources such as OpenStreetMap or Google Places) is not feasible. A common approach to evaluate clusterings when ground truth is absent is to use an internal cluster validity index (CVI). 
%CVIs include common indices like the Silhouette score~\cite{rousseeuw1987silhouettes}, the Dunn Index~\cite{dunn1973fuzzy}, and the Calinski-Harabasz criterion~\cite{calinski1974dendrite}. 
CVIs include common indices like the Silhouette score, the Dunn Index, and the Calinski-Harabasz criterion (see Arbelaitz ~\cite{arbelaitz2013extensive} for an overview of these techniques and references therein). Recent work recommends validation using multiple CVIs, as they each score different aspects of a clustering such as the ratio of inter- to intra-cluster distances, sum of squares distance to centroid, or graph-theory scores based on similarity~\cite{arbelaitz2013extensive}. 
We do not believe scores are informative for intrinsic POI evaluation, as most of these CVIs operate on unrealistic assumptions (e.g. symmetry or convexity of cluster shape, a notion of minimal variance, the existence of a centroid or medoid, etc.). Contrary to these widespread concepts, we do not assume that a cluster of exemplars representing an intrinsic POI will maintain some hyper-spherical or -elliptical shape. 
Indeed, there are a number of features within a geographical area that may be considered POIs, yet inevitably exhibit arbitrary shapes (e.g. buildings, parks, gathering areas, etc.) and manifest at varying densities (e.g. a busy intersection that is small and concentrated in exemplar density vs. a parking lot that is large and more uniform in density). 
Following the advice of Guyon and Luxburg {\em et al.}~\cite{guyon2009clustering, von2012clustering}, we evaluate the efficacy of the framework in the context of its end-use. We use an {\em external validation} where ``truth" can be defined a priori over simulated data, enabling a direct evaluation of intrinsic POIs against ``truly interesting'' regions, while ensuring the latent patterns in the generated data mimic the real geospatial dynamics of cars and pedestrians over a region. 

%Alternative means of evaluation rely on synthetic data generated a mixture of distributions to assess the statistical performance. While evaluation studies related to the statistical properties of the theoretical cluster tree are certainly valid research efforts, such studies are utterly unable to evaluate the {\em usefulness} of a clustering solution; the usefulness of a clustering algorithm can only be evaluated on a per-application basis~\cite{von2012clustering}. This perspective particularly applies to the current research efforts on POI discovery---the complexity of ``real-world'' traffic scenarios are too complex to be modeled sufficiently well from purely statistical point of view, i.e. object positions and times drawn by statistical distributions may not correspond with behaviors seen by objects moving in a geospace. 
\subsection{Generating synthetic data}
To generate synthetic data for evaluation, we turn to the Simulation of Urban MObility (SUMO) software~\cite{SUMO2012}. SUMO is an open source traffic simulation system capable of generating trajectories of many objects of multiple modalities (e.g. car, truck, person, plane, etc.). Given a shapefile that defines avenues for travel (e.g., a road network, a map of footpaths within a university campus, or the floor plan of a mall or large building), SUMO is able to generate trajectories following the avenues provided. Default parameter settings generate traffic and trajectories in ways that satisfy their measured physical properties have been shown to be incredibly accurate~\cite{SUMO2012}. We use SUMO to generate two simulations of both pedestrian and vehicular traffic under different geographical areas: an  urban region having a mixture of vehicle and pedestrian traffic (the area surrounding The Ohio State University (OSU)), and a suburban area where pedestrian traffic is more prominent (the area surrounding Wright State University (WSU)).
Details about the simulation, the simulation data used in this paper, and the code that produced the resulting evaluation are all publicly available and reproducible online.\footnote{See the following for simulation details: <Anonymized for review purposes.>} The (RSL) cluster tree framework itself is part of a larger open source effort by the author.\footnote{See the following package: <Anonymized for review purposes.>} 

\subsubsection*{Simulation configuration:}
SUMO requires every object to have a {\it trip} defined by departure and destination {\it nodes}, which SUMO refers to as {\it junctions}. Junctions are connected by edges representing a possible travel path. Given a file containing the trip definitions of every object, SUMO dynamically generates {\it routes}, or sequences of edges the object travels along to get from departure junction $A$ to its destination junction $B$. We leave nearly all simulation parameters at their default settings, only modifying simulation length and arrival parameters (binomially distributed arrivals) to generate pedestrian and vehicle demand. 

Because pedestrian traffic within unrestricted and indoor areas may constitute intrinsic POIs in a realistic setting, and because SUMO can generate only outdoor pedestrian traffic, we extended SUMO to simulate {\em indoor} pedestrian traffic as well. Figure~\ref{fig:sumo_pic} illustrates how this extension interplays with vehicular traffic generated by SUMO.\footnote{See <Anonymized for review purposes.>} Shapefiles denoting the location of buildings are first loaded into SUMO (the peach colored regions in Figure~\ref{fig:sumo_pic} inlet). Then, within the shapefile, a random number of pedestrian-only junctions are generated within the building and registered to nearby pedestrian-only edges (such as sidewalks). 
If a generated track is labeled as a pedestrian and its trip includes a junction contained within the building region (Figure~\ref{fig:sumo_pic}; lower right inlet), the pedestrian undergoes a random walk {\em within} the junctions generated in the building. This random walk is emulated by choosing a random ordered subset of the generated junctions for a random amount of time. The pedestrian visits these interior junctions and then travels to an `exit junction' attached to the building polygon, continuing along the original (outdoor) route generated by SUMO.
\subsubsection*{Defining truth:} 
Recall that intrinsic POIs are inferred by exemplars representing the specific mobility pattern of interest. With both vehicular and more realistic pedestrian demand generated, the next step in data generation is to define an aggregation function to extract meaningful exemplars. To give a concrete use-case of the proposed framework, we align our experiment with much of the applied literature related to this topic~\cite{zhou07, palma08, zheng2015trajectory} and extract exemplars representing the ``stay points'' of an object. A stay point is a position where objects have stopped or significantly slowed down. Extracting such points from simulated SUMO data is trivial, as the true speed of any traveling object is known at any given time. For pedestrian traffic, we extract trajectory points where pedestrians stopped moving. For vehicular traffic, we extract either a) the points where the vehicles stopped moving or b) the slowest point in a vehicle braking sequence using SUMOs exported braking signals, whichever is available. From these stay points (exemplars), we next establish a mapping between each exemplar and its presence within a ``true" intrinsic POI, allowing external validation. Since exemplars represent object stopped moving, a natural definition of an intrinsic POI is an assignment defined by the mechanism causing such objects to stop. Specifically, we define a building that pedestrians stop within as a ``true" intrinsic POI, as this is very natural and useful grouping.
We follow a similar pattern for vehicular traffic, assigning exemplars a common label if stopped at identical intersections, stop signs or stop light, or other junctions. This mechanistic assignment of creating ``true" intrinsic POIs has the benefit of not only being tractable (in the sense that SUMO provides this information directly), but also being {\em semantically meaningful} in the sense that the mechanisms encouraging objects to stop moving {\it are intrinsic to the geospace}. 
\begin{figure}
 	\includegraphics[width=0.48\textwidth, height=4cm]{sumo_fixed}
    \caption{Top-level view of extending SUMO to support indoor pedestrian traffic. 
    Shapefiles defining buildings are loaded into SUMO and registered as junction. 
    If pedestrian-track visits an attached junction during a trip, the simulator chooses
    ordered random set of junctions to follow within the building, exiting after a random period of time.}
    \label{fig:sumo_pic}
\end{figure}

 \subsection{Experimental Design}
 To evaluate the fidelity of the POIs extracted by the proposed framework under multiple settings, we run SUMO simulations over the OSU and WSU geospaces with parameter settings reflecting differences between the two regions. These settings are shown in Table~\ref{tab:table_1}. The OSU geospace covers a smaller area, has an equal mix of vehicles and pedestrians, and nearly three times as many buildings. The OSU geospace also has a larger number of roadways and traffic intersections where intrinsic POIs involving vehicles may materialize. Being within the main campus, the WSU geospace has a larger proportion of pedestrian traffic, with few roadways for vehicles to traverse and smaller number of buildings pedestrians may visit. 
 %The differences between OSU and WSU give us an opportunity to evaluate how well the proposed approach can extract intrinsic POI in two diverse regions. 
 Figures~\ref{fig:osu}(a) and~\ref{fig:wsu}(a) show what this SUMO generated POIs labeling creates for the OSU and WSU campus areas, respectively. 
 Qualitatively, examination of these clusters appear to be reasonable labels of intrinsic POIs. For example, the clusters representing ``true" POIs across OSU in Figure~\ref{fig:osu}(a) finds buildings surrounding the OSU oval quad, particular locations on the ring road around the quad (which tend to be busy OSU intersections for both vehicles and pedestrians), and parking lots around the OSU recreation builds west of the oval to represent POIs. 
 Across WSU in Figure~\ref{fig:wsu}(a), the truth POIs represent each of the major buildings around the campus, with particularly complex, separate areas of movement in WSU's large student union (the yellow points in the large building in the lower left part of the figure). 
 %Thus, these locations are subsequently colored by either the junction at which SUMO recorded the track as having stopped moving (in the vehicular case) or the building the pedestrian traffic is recorded within. We labeled such clusters as ``true" intrinsic POI for our subsequent analysis. Note that, unlike supervised validation, there is no distinction between a 'testing' and a 'truth' data set---both the SUMO generated labels and input set for every clustering algorithm testing uses the same data set. 

% $\sim Bin(1,\frac{1}{5})$$\sim Bin(5, p = \frac{1}{10})$
 %% Table of 3 simulation statistics and parameter settings
\def\tabularxcolumn#1{m{#1}}
\vspace*{-0.085cm}
\begin{table}
\caption{SUMO Simulation Parameters}
	\begin{center}\label{tab:1}
 	\begin{tabularx}{0.48\textwidth} {|| X | X | X | X | X | X | @{}m{0pt}@{} ||} 
 		\hline
 		Region & \# Buildings & \# Veh. & \# Ped. & Region size& Sim. Length  & \\ 
 		\hline\hline
 		OSU & 70 & 2,933 & 2,935 & 342km$^2$  & {\centering 8 hours} & \\ [2ex]
 		\hline
		WSU & 26 & 2,050 & 4,327 & 461km$^2$ & {\centering 6 hours} & \\ [2ex]
 		\hline
 	\end{tabularx}
	\end{center}
	\label{tab:table_1}
\end{table}

\begin{figure*}
\centering
	%% --- OSU Truth Solution ---
	\renewcommand{\thesubfigure}{a}
	\subcaptionbox{``True'' POIs}{
		\includegraphics[width=0.48\textwidth, height=5.55cm]{osu_truth}
	}%
	\hfill
	%% --- OSU Stable Solution ---
	\renewcommand{\thesubfigure}{b}
	\subcaptionbox{Inferred intrinsic POIs}{
		\includegraphics[width=0.48\textwidth, height=5.55cm]{osu_stable}
	}%
	\caption{Intrinsic POI comparison, OSU}
	\label{fig:osu}
\end{figure*}

%% WSU pictures single column
\begin{figure}
	\centering
	%% --- WSU Truth Solution ---
	\renewcommand{\thesubfigure}{c}
	\subcaptionbox{``True'' POIs}{
		\includegraphics[width=0.227\textwidth, height=4.85cm]{wsu_truth}
	}%
	\hfill
	%% --- WSU Stable Solution ---
	\renewcommand{\thesubfigure}{d}
	\subcaptionbox{Inferred intrinsic POIs}{
		\includegraphics[width=0.227\textwidth, height=4.85cm]{wsu_stable}
	}%
	\caption{Intrinsic POI comparison, WSU}
	\label{fig:wsu}
\end{figure}


%	
%	\subfloat[WSU] {
%		\includegraphics[width=0.15\textwidth]{wsu_truth}
%	\label{fig:wsu_truth}} 
%	%\caption{Synthetic ``truth" data generated by SUMO}
%%	\label{fig:truth_data}
%	

%\begin{figure}
%	\centering
%	
%	%% --- OSU Truth Solution ---
%	\subfloat[][OSU]{\includegraphics[width=0.35\textwidth]{osu_truth}\label{fig:osu_truth}}
%	
%	%% --- OSU Stable Solution --- 
%	\subfloat[OSU] {
%		\includegraphics[width=0.35\textwidth]{osu_stable}
%	\label{fig:osu_sol}}
%	
%	%% --- WSU Truth Solution ---
%	\subfloat[WSU] {
%		\includegraphics[width=0.15\textwidth]{wsu_truth}
%	\label{fig:wsu_truth}} 
%	%\caption{Synthetic ``truth" data generated by SUMO}
%%	\label{fig:truth_data}
%	
%	
%	%\centering
%	%% --- WSU Stable Solution ---
%	\subfloat[WSU] {
%		\includegraphics[width=0.15\textwidth]{wsu_stable}
%	\label{fig:wsu_sol}} 
%	%\caption{Points of interest inferred from the proposed framework}
%%	\label{fig:sol_data}
%\end{figure}

%\begin{figure*}
%	\centering
%	\subfloat[OSU] {
%		\includegraphics[width=0.4\textwidth]{osu_stable}
%	\label{fig:osu_sol}}
%	\subfloat[WSU] {
%		\includegraphics[width=0.27\textwidth]{wsu_stable}
%	\label{fig:wsu_sol}} 
%	\caption{Points of interest inferred from the proposed framework}
%	\label{fig:sol_data}
%\end{figure*}

%\begin{figure*}[htp]
%  \centering
%  \subfigure[Assigning truth labels: view of the SUMO-GUI]{\includegraphics[width=0.49\textwidth]{truth_sol}}
%  \subfigure[The resulting truth data generated by SUMO]{\includegraphics[width=0.49\textwidth]{stable_sol}}%\quad
% \caption{Assigning truth labels from SUMO}
%\label{fig:truth}
%\end{figure*}
\subsubsection*{Evaluation Measures:} 
 As discussed at the beginning of this section, the unsupervised nature of intrinsic POI discovery make it difficult to carry out a meaningful evaluation of POI discovery methods using {\em internal} (not requiring `truth' labels) validation measures. 
 Instead, we consider a multifaceted approach: an {\em external}, quantitative evaluation of whether the intrinsic POIs discovered aligns with SUMO generated POIs using the well-known Adjusted Rand Index (ARI)~\cite{hubert1985comparing}, and qualitative evaluation of the quality of the intrinsic POIs our approach unearths as compared to the ``true" intrinsic POIs as defined above. 
 The Rand-family of indices were chosen due to their transparency and simplicity---although, whereas the traditional RI measures the proportion of pairwise agreements between two partitions, the ARI also adjusts the score based on the expected value of agreements under the null hypothesis that the agreements were completely random, and thus is what we report. 
 % We also evaluated the results with the Fowlkes-Mallows index~\cite{ramirez2010probabilistic} and the normalized complement of the Variation of Information~\cite{meilua2003comparing}, but these results are omitted for the sake of compactness as the relative performance and resulting discussion remain the same for the ARI results. 

\subsubsection*{Algorithms Compared:} We further compare the fidelity of the intrinsic POIs extracted by the proposed framework against other clustering algorithms commonly used for POI discovery from trajectories. We either downloaded the implementation of, or implemented ourselves, a number of these algorithms for comparison. Aside from RSL, the selected methods includes the well-known density-based algorithms DBSCAN~\cite{ester1996density} and OPTICS~\cite{ankerst1999optics}, the widespread hierarchical algorithms single linkage (SL), average linkage (AL), and wards criterion (WL)~\cite{murtagh2014ward}, along with the partitioning-like algorithms $k$-means and CLARA~\cite{clara}. These algorithms were chosen due to their relevance to this problem, wide-spread availability, known success in the clustering world. 

\subsubsection*{Parameter Settings:} 
\label{sec:params} Clustering algorithms generally require parameter-tuning in order to `fit' to a given data set, but the number and semantics of these parameters often changes with the algorithm used, leaving comparisons between parameter settings difficult. 
Although most hierarchical algorithms carry no free parameters to create a (hierarchical) {\em set of solutions}, they do require either a threshold value ($h$) or the exact number of clusters to extract ($k$) to be specified to extract a `flat' clustering. Similarly, $k$-means and CLARA also require $k$ to be specified a priori. Because the $k$ parameter has the same interpretation in multiple algorithms, we will use $k$ to refer to {\em the number of clusters extracted}. Density based algorithms have multiple parameters with interpretations compared to the aforementioned algorithms. For example, DBSCAN requires a {\it minimum} cluster size parameter $\mathit{minPts}$ and a distance (or `scale') threshold $\epsilon$ to be set. OPTICS, often cited as  extension to DBSCAN, is an ordering algorithm that---given a parameter setting for $\mathit{minPts}$---can be be used to extract either a flat, DBSCAN-like cluster extraction or a simplified hierarchy using a either the a distance threshold $\epsilon'$ or a reachability-based threshold $\xi$, respectively. The DBSCAN-like cluster extraction is reported here. RSL requires the setting of $\alpha$ and $k$, the former relating to scaling the connection radii used to connect components, and the latter to the saliency of cluster estimates. Note that in RSL, $k$ is more similar to the $minPts$ parameter in that it is a {\em minimum} neighborhood parameter. The number of clusters is automatically determined by optimized the defined relative excess of mass functional from Section \ref{sec:methodology}. 

Each algorithm reflects a large set of possible solutions over its parameter setting. Choosing a single parameter setting for evaluation would represent a source of possible {\em bias}. Rather, we employ a more comprehensive approach by comparing a wide range of parameter settings for each algorithm. To define these ranges, let $\texttt{seq}(x,y,s)$ denote the sequential range operator, skipping $s$ values in the sequence of integers from $x$ to $y$. For example, $\texttt{seq}(1,n,1) = \{1, 2, \dots, n\}$, and  $\texttt{seq}(1,n,i) = \{1, 1 + i, \dots, n - i, n\}$. 
For the hierarchical clustering algorithms (SL, AL, and WL) the number of flat clusters extracted $k$ is varied in the range $\texttt{seq}(2,n_t,1)$ where $n_t$ is the number of ``true" POIs assigned by SUMO. We see this as a reasonable strategy, as it gives a better view of how multiple levels extracted from the hierarchy matched the data set as well as how well the merge criterion (or linkage function) collectively captures the true POIs in the geospace. We use the same range to vary $k$ for the $k$-means and CLARA algorithms. The density based methods DBSCAN and OPTICS are evaluated by first varying $\mathit{minPts}$, and then (for each value of $minPts$) by varying the scale parameters $\epsilon$ and $\epsilon'$, respectively. Recall $\mathit{minPts}$ relates to a {\it minimum} neighborhood value that constitutes a cluster. Thus, and to allow the testing to be tractable, we set $\mathit{minPts}$ to reflect the possible sizes of the POIs, along the {\em quantiles} $q_{n_t} = \texttt{seq}(0.10,0.95,0.025)$ corresponding to the the number of exemplars per POI in the SUMO ``truth'' data. The distance thresholds $\epsilon$ for DBSCAN and $\epsilon'$ OPTICS are also varied along the quantiles $\texttt{seq}(0.01,0.20,0.01)$ of the pairwise distances computed over the data set. Since all density-based methods mark points that fall in areas of the data set not sufficiently dense as `noise' according to a scale parameter---leading to severe overfitting if not guided with a measure like stability---all density-based solutions were deemed only valid if at least $75\%$ of the data is classified with a non-noise label. Finally, the RSL also contains two parameters, a $k$ value, and an $\alpha$ parameter. We use Chaudhuri {\em et. al}'s analysis to determine how to set these. RSL was shown to have optimal rates of convergence when $\alpha \geq \sqrt{2}$, so we leave it at that constant value ($\sqrt{2}$). Similarly, the rate only holds for $k$ at least as large as $d \log(n)$, where $d$ is the dimensionality of the data set ($d=2$ in this case). After varying through the small set of $k$ values in a similar fashion as was performed for DBSCAN and OPTICS ($k \in q_{n_t} \forall k >= d \log(n)$). 
% it should be noted that the proposed framework defines a single clustering result by finding the most stable set of locals cuts in the empirically estimated cluster tree (covered in Section \ref{sec:methodology}.3).
In total, 2,196 and 1,995 cluster configurations were performed for the OSU and WSU simulations respectively, totalling 4,191 reported configurations.  

 \subsection{Validation Testing and Discussion}
 \begin{figure*}\label{fig:res}
\begin{multicols}{2}
    \includegraphics[width=\linewidth, keepaspectratio]{osu_results}\par 
    \includegraphics[width=\linewidth, keepaspectratio]{wsu_results}\par 
 \end{multicols}
 \vspace*{-0.475cm}
\caption{The distribution of Adjusted Rand Index (ARI) scores of various clustering algorithms (after varying free parameters). The orange line corresponds to the ARI of the proposed framework.}
\label{fig:res}
\end{figure*}

\subsubsection*{Qualitative comparison to truth:}
Figures~\ref{fig:osu} and~\ref{fig:wsu} compare the intrinsic POIs discovered by our framework
agains the simulation's ``true" POIs. Recall that points with low density are discarded as noise (not shown). Direct comparison of the true POIs defined by the simulation show clear similarities. Over the OSU simulation in Figure~\ref{fig:osu}(b), the framework recovers intrinsic POIs within buildings no matter its shape, the density, or closeness to other buildings. It also recovers intrinsic POIs over parking lots and street intersections around the OSU oval. Some buildings are decomposed into a collection of individual intrinsic POIs. For example, the eastern-most large campus building by the northeast corner of the oval contains three separate intrinsic POIs: one at its entrance by the road, another in the center of the building, and a third at its back entrance. Although these labels may not match what SUMO assigned, they are in some sense more natural, i.e. it's quite possible for large buildings to have dense, isolated areas of people movement.

Looking at the intrinsic POIs over the WSU dataset in Figure~\ref{fig:wsu}(b), we find each building in general is recovered as an intrinsic POI and align in shape compared to the shape of the ``true" POIs from Figure~\ref{fig:wsu}(a). We also note that the framework determines that some movement within buildings but covering very small areas were found not be significant enough be an intrinsic POI. Large buildings also showed further decomposition like the OSU simulation. For example, in the WSU student union (large building in the lower left corner of the figure) the framework defines intrinsic POI's at the center and two back exits from the building. 

\subsubsection*{Quantitative comparison to other approaches:}
The proposed intrinsic POI framework measured ARI scores of $0.966$ on the OSU data set and $0.922$ for the WSU data set. Note that this is not the maximum ARI of any RSL solution, but the ARI of the solution found using the highest predefined notion of stability, determined completely without {\em any} knowledge of the surrounding geographical area.  RSL performed consistently in terms of having low variability compared to other algorithm, with overall high similarity to the semantically driven SUMO assigned locations. Figure~\ref{fig:res} shows the distribution of the ARI for the algorithms we compared our method against with the parameter settings discussed in Section~\ref{sec:params}. The orange line corresponds with the ARI of the proposed framework, which compares favorably with best possible settings of other algorithms. Note that although DBSCAN (like others) performed well with {\it very specific} configurations of $\mathit{minPts}$ and $\eps$, the settings of these parameters is often not very intuitive in unsupervised scenarios where the truth is unknown (and thus external measures like ARI cannot be computed). Of the hierarchical algorithms, we see the impact of the linkage criterion used and how they are influenced by the `shape' of the true clusters. For example, SL clustering performed fairly well on the well separated WSU data set, but substantially lower on the more density-varied OSU data set. This is reflected in AL as well. $k$-means was able capture much of the true clustering structure with the right parameter settings for the WSU simulation (with max/mean ARI scores of $(0.92, 0.71)$), however exhibited degraded performance when the POIs were less separated  in OSU data set ($(0.61, 0.84)$). OPTICS, with a few specific parameter settings, performed well on the WSU data set, however again suffered on the more variable-scale OSU data set.
 % On a related Without a formally defined relationship between parameter settings and model-selection, and without {\bf a clearly specified problem to solve}, there is little useful knowledge to gain from ad hoc cluster analysis of , especially when the solution space is large. 
 

==> ClusterTree POIs/semisupervised.tex <==
% --------------------------------------------------------------------
% ---------------- SEMISUPERVISED POI DETECTION ------------------------
% --------------------------------------------------------------------

% \subsubsection{Semi-supervised clustering} %% <- was this meant to be taken out? If so feel free to delete, wasn't sure if that was intended
% %% Yes, Matt, I think we should save details on augmentation for an extended version to a journal. 
% %% This is good content, but it brings us away from this idea that intrinsic POIs are totally data driven,
% %% and this is preferable because it works in settings where we do not need a gazetteer or external knowledge.  Let's save this!!! 

% The framework proposed above is application {\em agnostic}; any aggregate function can be used to extract exemplars, and it can be applied to many situations where one learn something `interesting' from a meaningfully aggregated set of trajectory data. 
% %% Quote paraphrased from Dr. Garber
% Nonetheless, any approach that neglecting alternative sources of information lead to suboptimal discriminative power.  
% %The properties of the nonparametric model underlying the framework apply to higher-dimensional sets of data as well, although the curse of dimensionality does affect the rates of convergence. 
% Recalling the unsupervised measure of cluster quality may be reasonably quantified through the relative excess of mass\ref{eq:9}. Denote this measure of cluster stability for a particular cluster $C_i$ as $S(C_i)$. The optimal unsupervised clustering solution may be found by maximizing the following: 
% \begin{equation}\label{eq:10}
% 	\begin{aligned}
% 		& \underset{\delta_1, \dots, \delta_m}{\text{maximize}}
% 		& & J_U = \sum\limits_{i = 2}^k \delta_i S(C_i) \\
% 		& \text{subject to}
% 		& & \delta_i \in \{ 0, 1 \}, i \in \{2, \dots, k\}
% 	\end{aligned}
% \end{equation}
% An often used approach of incorporating domain-specific information is through the use of {\it instance-level constraints}. See Wagstaff et. al~\cite{wagstaff2002intelligent} for more details on this semi-supervised form of clustering. Briefly, instance-level constraints enable the user to input pairwise relationships between individual points in the data matching the users preliminary expectation about the clustering. These pairwise relationship manifest as positive, {\it should-link} and negative, {\it should-not-link} constraints, respectively. Such constraints act as a priority scheme, enabling the user to specify ahead of time whether any two given data points should be part of the same cluster (positive constraint), or in separate clusters (negative constraint). Denote the number of the instance-level constraints satisfied involving any given point $x_j$ as $\gamma(x_j)$, the optimal clustering solution with respect to such constraint is the one that maximizes: 
% \begin{equation}\label{eq:11}
% 	J_{SS} = \frac{1}{2n_c}\sum\limits_{j = 1}^{n} \gamma(x_j)
% \end{equation}
% where $n_c$ is the number of total constraints, and $n$ is the total number of data points. $n_c$ is multiplied by $2$ to adjust for the fact that each constraint represents a relationship between two points, so as to scale the result to the unit interval. 
% With a cost function defined that, if maximized, results in either an optimal unsupervised or semi-supervised solution, the question remains how to combine these solutions in a meaningful way, and how to practically compute the solution. Campello et. al ~\cite{campello2013framework} provide a flexible framework for selecting the optimal clustering solution from any given hierarchical tree representation of clusters, and in doing so allow any convex combination of equations \ref{eq:10} or \ref{eq:11}:
% \begin{equation}\label{eq:12}
% 	J = J_{U}\alpha + (1 - \alpha) J_{SS}
% \end{equation} 

% We consider the use of this framework in context of the theoretical cluster tree estimated using RSL, and with respect to the domain of our analysis. The tools, approaches, and intentions regarding the incorporation of problem-specific information for the purpose of location discovery from trajectory data is remarkably diverse. See any of ~\cite{}. Such an approach {\em conceptually} similar to that of the CB-SMOT algorithm~\cite{palma08}, where application-specific information is available in the form of topologically closed polygons in $\mathbb{R}^2$ representing {\em known} locations. 
% %Note that this does not discount the existence of {\em unknown} locations, which can be inferred from the data. 
% Consider the scenario one is given the input data set of spatial positions of preprocessed trajectory exemplars. Imagine setting positive instance-level constraints (see ~\cite{wagstaff2002intelligent} for more details on this) between all points (pairwise) that intersect any location known {\it a priori}. This explicitly constrains the cluster solution extracted such that, if there are any exemplars that intersect a specific location, all exemplary data points within that same location take priority over any unsupervised measure cluster quality, restricting the cluster solution such that points within the same location {\em must} be merged together as a POI, subject to any contradictory constraints. Note that this is essentially the idea behind the efforts of Alvares and Palma et. al~\cite{alvares07, palma08} with ``known stops.'' 
% The primary difference of this effort being that {\em the solution space is restricted to conform to the supplied statistical notion of a POI.} Simply, the domain-specific constraints change {\em which} flat cluster solution is optimal based on the intent of the application, how the overall [hierarchical] set of clustering solutions is restricted to the set of high-density clusters. This is an important requirement, as it reflects the pivotal difference between an arbitrarily picked or predetermined set of POIs and the set of intrinsic POIs extracted from the cluster tree. Consider the illustrative example data set and corresponding potential clustering configuration shown in Figure \ref{fig:ss_vs_un}. 
%  \begin{figure}\label{fig:ss_vs_un}
%  		\includegraphics[width=0.50\textwidth,keepaspectratio]{ss2}
%     	\caption{SUMO.}
%  \end{figure}
%  The clusters are represented as connected components to emphasize the linkage. In the top figure, the left (red) and right (green) clusters correspond intuitively to what the average person may consider as known`locations,' and such locations can be considered as disjoint from unknown locations (blue) through the use of constraints that use the geometry of known POIs (the two buildings buildings outlined in black) to constrain the results. The cluster in the bottom picture illustrates what may be deemed, having no other information available, a more `stable' clustering. In this example, the cluster configuration at the top matches with what a user might expect based on {\it a priori} information, however {\em the data suggests that there is more evidence supporting the existence of one high-density cluster.} With smaller data sets, these differences may be likely be to noise due to random chance, and thus insignificant; however, if more data were collected over time, large differences from {\em expected} and {\em observed} POI definitions constitute situations where the something interesting may be happening. For example, consider the scenario where one has access to surveillance data tracking the trajectories (and stay points) of hundreds or thousands of people within an urban environment. Temporary events that draw large crowds of people (e.g. concerts, sports events, celebration ceremonies, etc.) will inevitably create very high-density clusters, and such situations {\em are} POIs.          

%
% Campello et. al~\cite{campello2013density} provide a 
%
%Imagine an unsupervised measure of quality that measures this 
%
%
%
%to that aims to obtain an optimal ``flat'' clustering results by maximizing a given objective function $J$, which 
%
%
%
%
%\begin{mydef}  {\bf Cluster Stability}\\
%	The stability of a cluster $S(C)$ can be defined as follows:
%	$$S(C) = \sum_{x_j \in C_i} \Big{(}\frac{1}{\epsilon_{\text{min}} (x_j, C_i)} - \frac{1}{\epsilon_{\text{max}} (C_i)}\Big{)} $$
%\end{mydef}
%
% 
 
 

%Traditional approaches to doing this, such as single linkage, complete linkage, average linkage, UPGMA, and other methods proposed by Ward. 



%\subsection*{Semi-supervised Location Discovery} 
%In the previous sections, a fram
%
%In domain-specific contexts, it may be useful to inject some amount of 
% 
% % Brief introduction into what several people are doing in the field 
%A framework for mining frequent periodic patterns and of long-lived object trajectories to identify POIs was proposed by \cite{mamoulis2004mining}. 
%
%\section{Defining Intrinsic Points of Interest}

%% Matt, open the section with some discussion about what it means for a PoI to be intrinsic and why they should exist in a geospatial database. Basically an elboration of the paragraph in the intro.  After the discussion, we should have defined some properties about what an intrinsic PoI is. 
%% We can then say, based on the definition and properties we described, density base clustering seems like a very reasonable way to go. While density-based clustering has its own problems (as described next) recent developments in the notion of consistency (Hartigan's work) suggest how a late-breaking density based clustering method serves as a suitable starting point to define an intrinsic point of interest.



%The collection of stay points represent regions of the coordinate space (geospace) where objects were found to have significantly lower spatial and temporal change in distance. These points have particular semantic meanings attached to them--naturally, one might expect that when observing vehicular traffic under heavy road-traffic conditions, a vehicle tends to stop or slow significantly a junction points. Similarly 


%
%\subsection*{Semisupervised Extraction}
%Furthermore, we introduce an automated approach to injecting reasonable bias into a stability-based cluster extraction approach as a means semi-supervised clustering geospatial data when existing knowledge bases are available. 



==> semisupervised.tex <==
% --------------------------------------------------------------------
% ---------------- SEMISUPERVISED POI DETECTION ------------------------
% --------------------------------------------------------------------

% \subsubsection{Semi-supervised clustering} %% <- was this meant to be taken out? If so feel free to delete, wasn't sure if that was intended
% %% Yes, Matt, I think we should save details on augmentation for an extended version to a journal. 
% %% This is good content, but it brings us away from this idea that intrinsic POIs are totally data driven,
% %% and this is preferable because it works in settings where we do not need a gazetteer or external knowledge.  Let's save this!!! 

% The framework proposed above is application {\em agnostic}; any aggregate function can be used to extract exemplars, and it can be applied to many situations where one learn something `interesting' from a meaningfully aggregated set of trajectory data. 
% %% Quote paraphrased from Dr. Garber
% Nonetheless, any approach that neglecting alternative sources of information lead to suboptimal discriminative power.  
% %The properties of the nonparametric model underlying the framework apply to higher-dimensional sets of data as well, although the curse of dimensionality does affect the rates of convergence. 
% Recalling the unsupervised measure of cluster quality may be reasonably quantified through the relative excess of mass\ref{eq:9}. Denote this measure of cluster stability for a particular cluster $C_i$ as $S(C_i)$. The optimal unsupervised clustering solution may be found by maximizing the following: 
% \begin{equation}\label{eq:10}
% 	\begin{aligned}
% 		& \underset{\delta_1, \dots, \delta_m}{\text{maximize}}
% 		& & J_U = \sum\limits_{i = 2}^k \delta_i S(C_i) \\
% 		& \text{subject to}
% 		& & \delta_i \in \{ 0, 1 \}, i \in \{2, \dots, k\}
% 	\end{aligned}
% \end{equation}
% An often used approach of incorporating domain-specific information is through the use of {\it instance-level constraints}. See Wagstaff et. al~\cite{wagstaff2002intelligent} for more details on this semi-supervised form of clustering. Briefly, instance-level constraints enable the user to input pairwise relationships between individual points in the data matching the users preliminary expectation about the clustering. These pairwise relationship manifest as positive, {\it should-link} and negative, {\it should-not-link} constraints, respectively. Such constraints act as a priority scheme, enabling the user to specify ahead of time whether any two given data points should be part of the same cluster (positive constraint), or in separate clusters (negative constraint). Denote the number of the instance-level constraints satisfied involving any given point $x_j$ as $\gamma(x_j)$, the optimal clustering solution with respect to such constraint is the one that maximizes: 
% \begin{equation}\label{eq:11}
% 	J_{SS} = \frac{1}{2n_c}\sum\limits_{j = 1}^{n} \gamma(x_j)
% \end{equation}
% where $n_c$ is the number of total constraints, and $n$ is the total number of data points. $n_c$ is multiplied by $2$ to adjust for the fact that each constraint represents a relationship between two points, so as to scale the result to the unit interval. 
% With a cost function defined that, if maximized, results in either an optimal unsupervised or semi-supervised solution, the question remains how to combine these solutions in a meaningful way, and how to practically compute the solution. Campello et. al ~\cite{campello2013framework} provide a flexible framework for selecting the optimal clustering solution from any given hierarchical tree representation of clusters, and in doing so allow any convex combination of equations \ref{eq:10} or \ref{eq:11}:
% \begin{equation}\label{eq:12}
% 	J = J_{U}\alpha + (1 - \alpha) J_{SS}
% \end{equation} 

% We consider the use of this framework in context of the theoretical cluster tree estimated using RSL, and with respect to the domain of our analysis. The tools, approaches, and intentions regarding the incorporation of problem-specific information for the purpose of location discovery from trajectory data is remarkably diverse. See any of ~\cite{}. Such an approach {\em conceptually} similar to that of the CB-SMOT algorithm~\cite{palma08}, where application-specific information is available in the form of topologically closed polygons in $\mathbb{R}^2$ representing {\em known} locations. 
% %Note that this does not discount the existence of {\em unknown} locations, which can be inferred from the data. 
% Consider the scenario one is given the input data set of spatial positions of preprocessed trajectory exemplars. Imagine setting positive instance-level constraints (see ~\cite{wagstaff2002intelligent} for more details on this) between all points (pairwise) that intersect any location known {\it a priori}. This explicitly constrains the cluster solution extracted such that, if there are any exemplars that intersect a specific location, all exemplary data points within that same location take priority over any unsupervised measure cluster quality, restricting the cluster solution such that points within the same location {\em must} be merged together as a POI, subject to any contradictory constraints. Note that this is essentially the idea behind the efforts of Alvares and Palma et. al~\cite{alvares07, palma08} with ``known stops.'' 
% The primary difference of this effort being that {\em the solution space is restricted to conform to the supplied statistical notion of a POI.} Simply, the domain-specific constraints change {\em which} flat cluster solution is optimal based on the intent of the application, how the overall [hierarchical] set of clustering solutions is restricted to the set of high-density clusters. This is an important requirement, as it reflects the pivotal difference between an arbitrarily picked or predetermined set of POIs and the set of intrinsic POIs extracted from the cluster tree. Consider the illustrative example data set and corresponding potential clustering configuration shown in Figure \ref{fig:ss_vs_un}. 
%  \begin{figure}\label{fig:ss_vs_un}
%  		\includegraphics[width=0.50\textwidth,keepaspectratio]{ss2}
%     	\caption{SUMO.}
%  \end{figure}
%  The clusters are represented as connected components to emphasize the linkage. In the top figure, the left (red) and right (green) clusters correspond intuitively to what the average person may consider as known`locations,' and such locations can be considered as disjoint from unknown locations (blue) through the use of constraints that use the geometry of known POIs (the two buildings buildings outlined in black) to constrain the results. The cluster in the bottom picture illustrates what may be deemed, having no other information available, a more `stable' clustering. In this example, the cluster configuration at the top matches with what a user might expect based on {\it a priori} information, however {\em the data suggests that there is more evidence supporting the existence of one high-density cluster.} With smaller data sets, these differences may be likely be to noise due to random chance, and thus insignificant; however, if more data were collected over time, large differences from {\em expected} and {\em observed} POI definitions constitute situations where the something interesting may be happening. For example, consider the scenario where one has access to surveillance data tracking the trajectories (and stay points) of hundreds or thousands of people within an urban environment. Temporary events that draw large crowds of people (e.g. concerts, sports events, celebration ceremonies, etc.) will inevitably create very high-density clusters, and such situations {\em are} POIs.          

%
% Campello et. al~\cite{campello2013density} provide a 
%
%Imagine an unsupervised measure of quality that measures this 
%
%
%
%to that aims to obtain an optimal ``flat'' clustering results by maximizing a given objective function $J$, which 
%
%
%
%
%\begin{mydef}  {\bf Cluster Stability}\\
%	The stability of a cluster $S(C)$ can be defined as follows:
%	$$S(C) = \sum_{x_j \in C_i} \Big{(}\frac{1}{\epsilon_{\text{min}} (x_j, C_i)} - \frac{1}{\epsilon_{\text{max}} (C_i)}\Big{)} $$
%\end{mydef}
%
% 
 
 

%Traditional approaches to doing this, such as single linkage, complete linkage, average linkage, UPGMA, and other methods proposed by Ward. 



%\subsection*{Semi-supervised Location Discovery} 
%In the previous sections, a fram
%
%In domain-specific contexts, it may be useful to inject some amount of 
% 
% % Brief introduction into what several people are doing in the field 
%A framework for mining frequent periodic patterns and of long-lived object trajectories to identify POIs was proposed by \cite{mamoulis2004mining}. 
%
%\section{Defining Intrinsic Points of Interest}

%% Matt, open the section with some discussion about what it means for a PoI to be intrinsic and why they should exist in a geospatial database. Basically an elboration of the paragraph in the intro.  After the discussion, we should have defined some properties about what an intrinsic PoI is. 
%% We can then say, based on the definition and properties we described, density base clustering seems like a very reasonable way to go. While density-based clustering has its own problems (as described next) recent developments in the notion of consistency (Hartigan's work) suggest how a late-breaking density based clustering method serves as a suitable starting point to define an intrinsic point of interest.



%The collection of stay points represent regions of the coordinate space (geospace) where objects were found to have significantly lower spatial and temporal change in distance. These points have particular semantic meanings attached to them--naturally, one might expect that when observing vehicular traffic under heavy road-traffic conditions, a vehicle tends to stop or slow significantly a junction points. Similarly 


%
%\subsection*{Semisupervised Extraction}
%Furthermore, we introduce an automated approach to injecting reasonable bias into a stability-based cluster extraction approach as a means semi-supervised clustering geospatial data when existing knowledge bases are available. 


